PASS: Peer-Agreement based Sample Selection for training with Noisy Labels

The prevalence of noisy-label samples poses a significant challenge in deep learning, inducing overfitting effects. This has, therefore, motivated the emergence of learning with noisy-label (LNL) techniques that focus on separating noisy- and clean-label samples to apply different learning strategies to each group of samples. Current methodologies often rely on the small-loss hypothesis or feature-based selection to separate noisy- and clean-label samples, yet our empirical observations reveal their limitations, especially for labels with instance dependent noise (IDN). An important characteristic of IDN is the difficulty to distinguish the clean-label samples that lie near the decision boundary (i.e., the hard samples) from the noisy-label samples. We, therefore, propose a new noisy-label detection method, termed Peer-Agreement based Sample Selection (PASS), to address this problem. Utilising a trio of classifiers, PASS employs consensus-driven peer-based agreement of two models to select the samples to train the remaining model. PASS is easily integrated into existing LNL models, enabling the improvement of the detection accuracy of noisy- and clean-label samples, which increases the classification accuracy across various LNL benchmarks.

==> clothing1m_csv/clean.tex <==
epochs,PASS,SmallLoss
1,0.7116375,0.6768125
2,0.7275515625,0.6710625
3,0.7077984375,0.69046875
4,0.7405781250000001,0.72015625
5,0.75193125,0.70946875
6,0.7562625,0.7211875
7,0.754228125,0.71425
8,0.743596875,0.70003125
9,0.764990625,0.716375
10,0.76584375,0.71628125
11,0.7702078125,0.72790625
12,0.774178125,0.72215625
13,0.778246875,0.7379375
14,0.769059375,0.73240625
15,0.76899375,0.73090625
16,0.7638421875,0.736625
17,0.7818234375,0.742125
18,0.7766390625,0.738875
19,0.77424375,0.7244375
20,0.77923125,0.74834375
21,0.7667953125,0.73665625
22,0.7809703124999999,0.74534375
23,0.7784765625000001,0.74215625
24,0.782971875,0.74184375
25,0.7854984375,0.73415625
26,0.7784765625000001,0.7424375
27,0.8082046875000001,0.74965625
28,0.78211875,0.74721875
29,0.7988859375,0.74678125
30,0.7809046875,0.74546875
31,0.80180625,0.754
32,0.78028125,0.7540625
33,0.7878281250000001,0.757625
34,0.7846781250000001,0.746625
35,0.7819546875,0.73784375
36,0.7930781250000001,0.7504375
37,0.779953125,0.74534375
38,0.7795265625000001,0.7570625
39,0.7899609375,0.74225
40,0.7859250000000001,0.7524375
41,0.793865625,0.75196875
42,0.8005593750000001,0.77084375
43,0.8038734375,0.7654375
44,0.8197875000000001,0.7918125
45,0.8054484375000001,0.77359375
46,0.7988859375,0.77403125
47,0.803315625,0.76896875
48,0.8050875000000001,0.77684375
49,0.8043328125000001,0.77384375
50,0.802396875,0.77140625
51,0.8004281249999999,0.775125
52,0.807121875,0.77446875
53,0.808171875,0.77640625
54,0.814078125,0.7741875
55,0.8097468750000001,0.77659375
56,0.811059375,0.7703125
57,0.8129625,0.77646875
58,0.813815625,0.76934375
59,0.8085656250000001,0.77178125
60,0.8221171875000001,0.77696875
61,0.8105671875,0.76459375
62,0.813684375,0.7753125
63,0.813815625,0.77603125
64,0.8035125000000001,0.768375
65,0.8112890625000001,0.77340625
66,0.8116828125,0.7799375
67,0.8172609375000001,0.7756875
68,0.81020625,0.77871875
69,0.804825,0.779
70,0.81335625,0.78128125
71,0.8196234375,0.77890625
72,0.8182453125000001,0.780125
73,0.812634375,0.77478125
74,0.808828125,0.77915625
75,0.8208046875,0.7751875
76,0.819984375,0.782875
77,0.8211328125,0.77778125
78,0.8259890624999999,0.78521875
79,0.8203453125000001,0.786375

==> clothing1m_csv/f1.tex <==
epochs,PASS,SmallLoss
0,0.6863917713408,0.6827687183
1,0.6862857434496,0.6767522833
2,0.6918590723183999,0.6798771483
3,0.6855643703663999,0.6907072447
4,0.6930865562544,0.6994224939
5,0.701677077696,0.6978985245
6,0.7020312123888,0.7057251528
7,0.7075152545328001,0.6998379979
8,0.704510744112,0.7055346368
9,0.7146243438768001,0.7058329942
10,0.7183681221024001,0.7150097157
11,0.7163837084879999,0.7187430128
12,0.715813105392,0.714217813
13,0.7056620277840001,0.7170773652
14,0.7221606427728,0.7178012061
15,0.7177425939936,0.7183521779
16,0.7259797286784,0.7169722084
17,0.7190862715008,0.7141971518
18,0.7221514547519999,0.7224119203
19,0.7203897153936,0.7230264096
20,0.7201642073472,0.7227279011
21,0.7217687002176,0.7241472537
22,0.7300540611504001,0.712610093
23,0.723241652616,0.7131621728
24,0.7302428218512,0.723651918
25,0.7278029180352,0.7281497588
26,0.729202630464,0.7230852008
27,0.7406918132544,0.7285464098
28,0.7280325515232,0.7217812205
29,0.7351930608624,0.7257277825
30,0.7326843317135999,0.7268735822
31,0.735736101408,0.7255990393
32,0.732967147584,0.7191254532
33,0.7297857708624,0.73211416
34,0.7364440616400001,0.7280259863
35,0.728829614016,0.7331954735
36,0.7280665564032,0.7260972784
37,0.732572512056,0.7244935669
38,0.729034295472,0.7240682826
39,0.7349425600607999,0.729452465
40,0.7432590980304,0.7317314818
41,0.7341577053552,0.7403733382
42,0.746564368032,0.7423730448
43,0.7436783347056,0.7350771428
44,0.748065891888,0.743428743
45,0.7481242532736,0.7426447316
46,0.7488427662576,0.736443888
47,0.7447201950384,0.7428863021
48,0.7423960276656,0.7436459415
49,0.7407444480912,0.7415472164
50,0.7456431864672001,0.7403347396
51,0.7469723151072,0.7348937992
52,0.749833291872,0.7410845655
53,0.74589488568,0.739328924
54,0.7507974608064,0.7420231396
55,0.7467714620352001,0.7449103371
56,0.7503355462176,0.7399767366
57,0.7523521809552,0.7420876669
58,0.7454661675551999,0.7373448603
59,0.7436289012768,0.7444684695
60,0.7512506935919999,0.742509331
61,0.7508204074224,0.7462584833
62,0.7514104683456,0.744091198
63,0.748613833128,0.7278436984
64,0.7504900901568,0.7443723516
65,0.7534253056175999,0.7447085383
66,0.7498552222224,0.741023698
67,0.751548076776,0.7486974899
68,0.7530342914304,0.7446765445
69,0.7510651956864,0.7449476432
70,0.7461241474176,0.7414573805
71,0.7538502967632,0.7444515971
72,0.7468575021936,0.7411953891
73,0.7498082599056,0.7455266484
74,0.7524439995744,0.7432638778
75,0.7529431625856,0.7419166613
76,0.7495934622624,0.7456797984
77,0.7452761258880001,0.7475653963
78,0.750082751208,0.7424101268
79,0.7480391599296,0.7407056488

==> clothing1m_csv/precision.tex <==
epochs,PASS,SmallLoss
0,0.7016449722,0.7004962673
1,0.6882589145,0.7021021739
2,0.7027316114,0.6910284426
3,0.6874738178,0.6958322272
4,0.6943569507,0.7058239358
5,0.7069871077,0.7125143759
6,0.7055903267,0.7175886227
7,0.7117045292,0.7062404186
8,0.7105743986,0.7131796194
9,0.7192448593,0.7181439951
10,0.7219425593,0.723648598
11,0.7219399934,0.7271774175
12,0.7214344102,0.7236354227
13,0.7154232302,0.7257077424
14,0.7236324272,0.7261607276
15,0.72478322,0.7286898577
16,0.7240980478,0.7269545496
17,0.7212727148,0.7209815675
18,0.7272048702,0.7312330878
19,0.7236096636,0.7291465334
20,0.7202611465,0.7288232682
21,0.7304189455,0.7310902495
22,0.7348860195,0.7245731493
23,0.7295652296,0.7225322303
24,0.7300771159,0.7322785651
25,0.7312272501,0.7368216664
26,0.7297723626,0.729934314
27,0.7407406124,0.7351135091
28,0.7344465716,0.7319500954
29,0.7329233196,0.7354469661
30,0.7394384103,0.7365741184
31,0.7358302952,0.7345074062
32,0.7337221568,0.7294929338
33,0.7305057141,0.7342819233
34,0.7355775466,0.7323651126
35,0.7337386006,0.7401014407
36,0.7330280326,0.7395553704
37,0.7366300035,0.7370215279
38,0.7284400751,0.7333514016
39,0.7358250236,0.7390204629
40,0.7444038301,0.743350374
41,0.7383586249,0.7474690915
42,0.7471756699,0.748059576
43,0.7452307206,0.7412569496
44,0.7497039532,0.7509244976
45,0.7455000706,0.749715208
46,0.7515420085,0.7451567228
47,0.7485361434,0.7508994204
48,0.7404189624,0.7481651847
49,0.7405610624,0.7475781328
50,0.7461857128,0.748144413
51,0.7476566696,0.7439249073
52,0.7504526072,0.7497124231
53,0.7470244472,0.7445428727
54,0.7523345173,0.7465509019
55,0.7479173424,0.7481408033
56,0.7496975987,0.7453941774
57,0.7501967766,0.7489884046
58,0.7442435246,0.7448023956
59,0.7428470305,0.7506867623
60,0.7480599024,0.7465677384
61,0.7506017822,0.7502528295
62,0.7499616532,0.7499856611
63,0.7487006875,0.7402711062
64,0.7504554854,0.7513807549
65,0.7543169823,0.7531042368
66,0.7494400752,0.7472623291
67,0.7497598768,0.7520775114
68,0.754571907,0.7501587731
69,0.7503694522,0.7497603081
70,0.7496834385,0.7473804575
71,0.7535965194,0.7494398306
72,0.7498685044,0.7488199182
73,0.7540241325,0.7483240351
74,0.7521995331,0.750399555
75,0.7555590953,0.7488430787
76,0.7507468879,0.7500685471
77,0.7505523375,0.7530702013
78,0.7487839231,0.7482390646
79,0.748517483,0.7491151327

==> clothing1m_csv/precision_.tex <==
epochs,PASS,SmallLoss
0,0.708661421922,0.7004962673
1,0.6951415036449999,0.7021021739
2,0.7097589275139999,0.6910284426
3,0.694348555978,0.6958322272
4,0.7013005202070001,0.7058239358
5,0.7140569787769999,0.7125143759
6,0.712646229967,0.7175886227
7,0.718821574492,0.7062404186
8,0.7176801425860001,0.7131796194
9,0.7264373078930001,0.7181439951
10,0.729161984893,0.723648598
11,0.729159393334,0.7271774175
12,0.728648754302,0.7236354227
13,0.722577462502,0.7257077424
14,0.730868751472,0.7261607276
15,0.7320310522,0.7286898577
16,0.731339028278,0.7269545496
17,0.728485441948,0.7209815675
18,0.7344769189020001,0.7312330878
19,0.730845760236,0.7291465334
20,0.727463757965,0.7288232682
21,0.737723134955,0.7310902495
22,0.742234879695,0.7245731493
23,0.7368608818960001,0.7225322303
24,0.737377887059,0.7322785651
25,0.738539522601,0.7368216664
26,0.737070086226,0.729934314
27,0.748148018524,0.7351135091
28,0.741791037316,0.7319500954
29,0.740252552796,0.7354469661
30,0.746832794403,0.7365741184
31,0.743188598152,0.7345074062
32,0.741059378368,0.7294929338
33,0.737810771241,0.7342819233
34,0.7429333220659999,0.7323651126
35,0.7410759866059999,0.7401014407
36,0.7403583129260001,0.7395553704
37,0.743996303535,0.7370215279
38,0.735724475851,0.7333514016
39,0.743183273836,0.7390204629
40,0.751847868401,0.743350374
41,0.7457422111490001,0.7474690915
42,0.754647426599,0.748059576
43,0.7526830278059999,0.7412569496
44,0.757200992732,0.7509244976
45,0.752955071306,0.749715208
46,0.759057428585,0.7451567228
47,0.756021504834,0.7508994204
48,0.7478231520240001,0.7481651847
49,0.747966673024,0.7475781328
50,0.753647569928,0.748144413
51,0.755133236296,0.7439249073
52,0.757957133272,0.7497124231
53,0.754494691672,0.7445428727
54,0.759857862473,0.7465509019
55,0.7553965158239999,0.7481408033
56,0.757194574687,0.7453941774
57,0.7576987443659999,0.7489884046
58,0.751685959846,0.7448023956
59,0.750275500805,0.7506867623
60,0.755540501424,0.7465677384
61,0.758107800022,0.7502528295
62,0.757461269732,0.7499856611
63,0.756187694375,0.7402711062
64,0.757960040254,0.7513807549
65,0.761860152123,0.7531042368
66,0.756934475952,0.7472623291
67,0.757257475568,0.7520775114
68,0.76211762607,0.7501587731
69,0.757873146722,0.7497603081
70,0.757180272885,0.7473804575
71,0.7611324845940001,0.7494398306
72,0.7573671894439999,0.7488199182
73,0.761564373825,0.7483240351
74,0.7597215284309999,0.750399555
75,0.7631146862529999,0.7488430787
76,0.758254356779,0.7500685471
77,0.758057860875,0.7530702013
78,0.756271762331,0.7482390646
79,0.75600265783,0.7491151327

==> csv/clean.tex <==
id,epochs,FINE,PASS,SmallLoss
0,50,0.84116,0.44327800000000006,0.66368
1,51,0.66168,0.44492800000000005,0.66098
2,52,0.67572,0.44334400000000007,0.66758
3,53,0.6637,0.44393800000000005,0.66656
4,54,0.67574,0.444114,0.66804
5,55,0.67826,0.443674,0.66758
6,56,0.67798,0.44431200000000004,0.66258
7,57,0.67868,0.44444400000000006,0.6633
8,58,0.68186,0.44488400000000006,0.6618
9,59,0.68078,0.44437800000000005,0.66534
10,60,0.68118,0.444708,0.65798
11,61,0.68176,0.4439600000000001,0.66678
12,62,0.68142,0.44409200000000004,0.66832
13,63,0.67678,0.44354200000000005,0.66888
14,64,0.68156,0.44316800000000006,0.66124
15,65,0.68136,0.44453200000000004,0.66356
16,66,0.67692,0.44453200000000004,0.66224
17,67,0.67954,0.44433400000000006,0.6628
18,68,0.67632,0.44565400000000005,0.6727
19,69,0.68008,0.44554400000000005,0.66264
20,70,0.6741,0.44558800000000004,0.6621
21,71,0.67984,0.447832,0.65744
22,72,0.67856,0.44563200000000003,0.65944
23,73,0.67954,0.44583,0.66108
24,74,0.67672,0.44675400000000004,0.66028
25,75,0.67872,0.44761200000000007,0.66122
26,76,0.67696,0.44708400000000004,0.66582
27,77,0.67318,0.4470180000000001,0.65892
28,78,0.68106,0.448404,0.66752
29,79,0.6771,0.44825,0.6601
30,80,0.68062,0.44679800000000003,0.66116
31,81,0.67812,0.44792000000000004,0.65362
32,82,0.67782,0.448998,0.65842
33,83,0.6729,0.448558,0.66156
34,84,0.67036,0.44811800000000007,0.66142
35,85,0.67688,0.44853600000000005,0.65706
36,86,0.67906,0.447766,0.6599
37,87,0.67626,0.44424600000000003,0.66088
38,88,0.67084,0.44811800000000007,0.65936
39,89,0.67568,0.4494600000000001,0.65538
40,90,0.67098,0.450142,0.6561
41,91,0.6734,0.448316,0.65752
42,92,0.66048,0.449504,0.65502
43,93,0.67984,0.45031800000000005,0.65546
44,94,0.66836,0.44992200000000004,0.6517
45,95,0.66886,0.45029600000000003,0.6594
46,96,0.66746,0.44849200000000006,0.6521
47,97,0.66836,0.45012,0.65462
48,98,0.66826,0.452012,0.65242
49,99,0.66714,0.44939400000000007,0.65612
50,100,0.66774,0.45113200000000003,0.64906
51,101,0.66104,0.45181400000000005,0.65016
52,102,0.66778,0.45124200000000003,0.65288
53,103,0.6594,0.453134,0.65344
54,104,0.66248,0.45124200000000003,0.64974
55,105,0.65686,0.45045,0.64868
56,106,0.65888,0.45012,0.6526
57,107,0.66018,0.45262800000000003,0.65662
58,108,0.65668,0.45300200000000007,0.6525
59,109,0.6662,0.45155,0.65232
60,110,0.657,0.4525180000000001,0.65164
61,111,0.65704,0.453222,0.65508
62,112,0.6568,0.453266,0.65104
63,113,0.65574,0.45174800000000004,0.65578
64,114,0.66232,0.453508,0.65268
65,115,0.65554,0.45348600000000006,0.65552
66,116,0.66048,0.45447600000000005,0.65344
67,117,0.65386,0.453882,0.65264
68,118,0.65708,0.4512860000000001,0.65674
69,119,0.6575,0.45302400000000004,0.65366
70,120,0.66116,0.45408000000000004,0.6514
71,121,0.6557,0.45463000000000003,0.65856
72,122,0.65918,0.45555400000000007,0.658
73,123,0.65718,0.45410200000000006,0.6543
74,124,0.65408,0.45366200000000007,0.65226
75,125,0.65814,0.45324400000000004,0.65404
76,126,0.6583,0.45513600000000004,0.656
77,127,0.65722,0.4548940000000001,0.65394
78,128,0.65776,0.45507000000000003,0.654
79,129,0.66108,0.45465200000000006,0.6522
80,130,0.65736,0.45529000000000003,0.6458
81,131,0.65666,0.45636800000000005,0.65236
82,132,0.66178,0.4536180000000001,0.65142
83,133,0.65332,0.45612600000000003,0.65348
84,134,0.6556,0.45683,0.65548
85,135,0.65318,0.45691800000000005,0.6539
86,136,0.65302,0.455576,0.65626
87,137,0.65592,0.45612600000000003,0.6513
88,138,0.65354,0.45771000000000006,0.65528
89,139,0.65604,0.45716000000000007,0.65488
90,140,0.65534,0.457116,0.6539
91,141,0.65718,0.45654400000000006,0.65204
92,142,0.6567,0.45562,0.65278
93,143,0.66046,0.4574020000000001,0.65454
94,144,0.6535,0.4587,0.6497
95,145,0.6542,0.4576,0.65206
96,146,0.65342,0.45859000000000005,0.6489
97,147,0.65558,0.457776,0.65268
98,148,0.6561,0.45793000000000006,0.6518
99,149,0.66224,0.457116,0.65422
100,150,0.65734,0.458876,0.65308
101,151,0.65654,0.460042,0.6553
102,152,0.65882,0.460108,0.65504
103,153,0.65966,0.460504,0.6559
104,154,0.6586,0.45975600000000005,0.6585
105,155,0.65752,0.4609440000000001,0.65632
106,156,0.65868,0.46103200000000005,0.65578
107,157,0.65954,0.461318,0.65856
108,158,0.6603,0.4616700000000001,0.65832
109,159,0.66032,0.46151600000000004,0.65784
110,160,0.66024,0.46191200000000004,0.65714
111,161,0.66094,0.4616700000000001,0.6569
112,162,0.6597,0.46233,0.65658
113,163,0.65998,0.46208800000000005,0.65956
114,164,0.65932,0.462924,0.6575
115,165,0.66092,0.462616,0.65962
116,166,0.66034,0.46354,0.65754
117,167,0.65922,0.46266,0.65824
118,168,0.65978,0.46285800000000005,0.65704
119,169,0.6601,0.4629020000000001,0.65624
120,170,0.65956,0.46288000000000007,0.65744
121,171,0.66046,0.46343000000000006,0.65632
122,172,0.65934,0.463716,0.65776
123,173,0.65962,0.46314400000000006,0.658
124,174,0.65946,0.46354,0.65802
125,175,0.6593,0.46446400000000004,0.65784
126,176,0.6596,0.46369400000000005,0.65818
127,177,0.66012,0.46446400000000004,0.6571
128,178,0.65894,0.46446400000000004,0.65738
129,179,0.65912,0.46450800000000003,0.65926
130,180,0.65864,0.46428800000000003,0.6576
131,181,0.65834,0.46530000000000005,0.65776
132,182,0.65832,0.46393600000000007,0.65704
133,183,0.65862,0.46464000000000005,0.65764
134,184,0.65924,0.46514600000000006,0.65832
135,185,0.6582,0.465058,0.65592
136,186,0.6588,0.46459600000000006,0.65724
137,187,0.65964,0.4646620000000001,0.65622
138,188,0.6586,0.46483800000000003,0.65678
139,189,0.65882,0.46519000000000005,0.65692
140,190,0.65924,0.465102,0.65696
141,191,0.65908,0.46486,0.65668
142,192,0.65894,0.466092,0.6569
143,193,0.65882,0.465542,0.6576
144,194,0.65938,0.46648800000000007,0.6564
145,195,0.658,0.465718,0.65622
146,196,0.65926,0.46646600000000005,0.65712
147,197,0.65916,0.466752,0.65666
148,198,0.65964,0.46679600000000004,0.65736
149,199,0.65944,0.467434,0.65614
150,200,0.6591,0.46651000000000004,0.65722
151,201,0.65836,0.466664,0.65676
152,202,0.65808,0.46708200000000005,0.65602
153,203,0.66,0.46723600000000004,0.65626
154,204,0.65888,0.46706000000000003,0.657
155,205,0.65928,0.46752200000000005,0.65686
156,206,0.65966,0.46774200000000005,0.65736
157,207,0.65964,0.46761,0.65618
158,208,0.6588,0.46794,0.6545
159,209,0.6585,0.46756600000000004,0.6561
160,210,0.658,0.46723600000000004,0.65536
161,211,0.65864,0.46741200000000005,0.65608
162,212,0.65932,0.467874,0.65708
163,213,0.6583,0.46763200000000005,0.657
164,214,0.65846,0.467874,0.65676
165,215,0.65926,0.46734600000000004,0.65554
166,216,0.6581,0.468094,0.65656
167,217,0.65728,0.46831400000000006,0.657
168,218,0.65962,0.4682700000000001,0.65626
169,219,0.66006,0.468468,0.65576
170,220,0.65804,0.468424,0.6559
171,221,0.65836,0.46871,0.65594
172,222,0.6587,0.4686,0.65704
173,223,0.65834,0.468402,0.65642
174,224,0.65842,0.46890800000000005,0.65478
175,225,0.65964,0.468534,0.65706
176,226,0.65818,0.46862200000000004,0.65526
177,227,0.65802,0.46820400000000006,0.6571
178,228,0.65932,0.4689960000000001,0.655
179,229,0.65728,0.46930400000000005,0.65598
180,230,0.65886,0.46930400000000005,0.65594
181,231,0.65818,0.4696120000000001,0.65636
182,232,0.6575,0.46967800000000004,0.65692
183,233,0.6578,0.469216,0.6558
184,234,0.65818,0.469084,0.6557
185,235,0.65856,0.46959000000000006,0.65558
186,236,0.65822,0.46978800000000004,0.6558
187,237,0.65888,0.46985400000000005,0.65596
188,238,0.65872,0.46923800000000004,0.6558
189,239,0.65944,0.469876,0.65524
190,240,0.65958,0.46967800000000004,0.65708
191,241,0.65882,0.46956800000000004,0.6552
192,242,0.6587,0.47088800000000003,0.65588
193,243,0.6583,0.46992000000000006,0.65576
194,244,0.65858,0.47106400000000004,0.65734
195,245,0.6586,0.470536,0.65662
196,246,0.65912,0.4701620000000001,0.65652
197,247,0.65934,0.4702280000000001,0.65606
198,248,0.65694,0.47055800000000003,0.65724
199,249,0.65892,0.471042,0.65664
200,250,0.65932,0.47040400000000004,0.65698
201,251,0.65816,0.470866,0.65564
202,252,0.65812,0.4707780000000001,0.65576
203,253,0.6591,0.471482,0.65578
204,254,0.65852,0.47124000000000005,0.65464
205,255,0.65992,0.47172400000000003,0.6563
206,256,0.65736,0.4713280000000001,0.6566
207,257,0.65962,0.47185600000000005,0.65612
208,258,0.65822,0.47190000000000004,0.65642
209,259,0.65962,0.472494,0.65642
210,260,0.65916,0.47168000000000004,0.65568
211,261,0.65984,0.472208,0.65544
212,262,0.65906,0.471636,0.6567
213,263,0.65918,0.4726700000000001,0.65672
214,264,0.65904,0.472076,0.65726
215,265,0.65944,0.47223000000000004,0.65654
216,266,0.65888,0.47181200000000006,0.65672
217,267,0.65946,0.47251600000000005,0.65664
218,268,0.6601,0.472274,0.65732
219,269,0.66012,0.472142,0.65706
220,270,0.66004,0.472384,0.65724
221,271,0.6611,0.47245000000000004,0.65786
222,272,0.66052,0.473308,0.6565
223,273,0.66046,0.472736,0.6584
224,274,0.66064,0.473924,0.65662
225,275,0.6599,0.47313200000000005,0.65626
226,276,0.65878,0.47357200000000005,0.65748
227,277,0.65986,0.47368200000000005,0.65748
228,278,0.66008,0.473902,0.65702
229,279,0.66032,0.47423200000000004,0.65608
230,280,0.6603,0.47363800000000006,0.6574
231,281,0.6592,0.473968,0.65686
232,282,0.65986,0.47379200000000005,0.65778
233,283,0.65944,0.47379200000000005,0.65726
234,284,0.66026,0.47372600000000004,0.65656
235,285,0.6598,0.47355,0.65858
236,286,0.65994,0.4743200000000001,0.65688
237,287,0.65954,0.474078,0.65826
238,288,0.66032,0.47454,0.65806
239,289,0.65738,0.47429800000000005,0.65788
240,290,0.65894,0.4743200000000001,0.65748
241,291,0.65946,0.47454,0.65626
242,292,0.65944,0.4752,0.65742
243,293,0.65892,0.47533200000000003,0.65726
244,294,0.66058,0.47509000000000007,0.65618
245,295,0.65916,0.475486,0.65512
246,296,0.65918,0.47522200000000003,0.65672
247,297,0.65956,0.475156,0.65628
248,298,0.65966,0.47612400000000005,0.6569
249,299,0.66176,0.4757060000000001,0.6566
250,300,0.65984,0.47590400000000005,0.65734

==> csv/f1.tex <==
epochs,FINE,PASS,SmallLoss
50,0.651564233,0.8639118461,0.7603369483
51,0.687575284,0.8656233308,0.7555153816
52,0.7248125159,0.8630582597,0.7554439877
53,0.7392473678,0.8646236566,0.7586395683
54,0.7367128176,0.8650903911,0.7587101238
55,0.7485922849,0.8648079294,0.7608923531
56,0.7503319104,0.8665104289,0.7584033669
57,0.7521286787,0.8658656202,0.7587270573
58,0.748827243,0.8655288722,0.7578083226
59,0.748492592,0.8659227884,0.7578166858
60,0.7514583087,0.8664324054,0.7536635027
61,0.7551878232,0.8661081446,0.7607259736
62,0.7520852654,0.8662148195,0.760857709
63,0.7522497348,0.8649222224,0.7589545336
64,0.7549764698,0.8635202003,0.7582755205
65,0.751141095,0.8665849296,0.7571484907
66,0.7554922532,0.8668059071,0.758383287
67,0.7535501077,0.8662261315,0.7582261028
68,0.7557058531,0.867246904,0.7612012533
69,0.7566650862,0.8675188259,0.7590870456
70,0.7544023204,0.8673923906,0.7599202038
71,0.7553262272,0.8708259662,0.7596824836
72,0.7562108737,0.8675749921,0.7586193757
73,0.7577562105,0.8679771899,0.7607915853
74,0.7582381767,0.869558014,0.7573829466
75,0.7545812023,0.8696952509,0.7614237818
76,0.7586621317,0.8698007154,0.7587758133
77,0.7564918938,0.8697698218,0.760649824
78,0.7566497528,0.8705497999,0.7589780219
79,0.7588442117,0.8714759286,0.7615004005
80,0.7575405103,0.8690788888,0.7589821871
81,0.7564241433,0.8718947285,0.7588229439
82,0.7562762728,0.8724107278,0.7613220488
83,0.7545226442,0.8725730373,0.7602374827
84,0.7550248511,0.8717667146,0.7604665083
85,0.7573196351,0.8725041273,0.7594813731
86,0.7568078045,0.8711475727,0.7598375243
87,0.7579891771,0.8674518087,0.7608186885
88,0.7558785202,0.8720749619,0.7610525843
89,0.7552986801,0.8735927179,0.7609963513
90,0.7584877675,0.8738790698,0.7605245103
91,0.7572031088,0.8714626445,0.7592500133
92,0.757321944,0.8727629319,0.7580804253
93,0.7551566689,0.8736821886,0.7607361479
94,0.7607290462,0.8728395689,0.7603950193
95,0.7568452616,0.873437668,0.7605088361
96,0.756926386,0.8717940534,0.7610003218
97,0.7613111752,0.8725797837,0.7611138952
98,0.7612048255,0.8751518037,0.7634977519
99,0.7595325556,0.8725066559,0.7610996951
100,0.7584930445,0.8735901941,0.7606719853
101,0.7587156966,0.8756309617,0.7613738497
102,0.7593236881,0.8749872376,0.7608347529
103,0.7610609506,0.8765440893,0.762721521
104,0.7628391397,0.8737142125,0.7634601464
105,0.7585400135,0.8732599954,0.7625246189
106,0.7577415063,0.8731071484,0.7645938817
107,0.7602067001,0.8766334339,0.7610488501
108,0.7565476068,0.8767026577,0.7660831307
109,0.7581865891,0.8750267641,0.7631470974
110,0.7596934792,0.876334545,0.7595312332
111,0.7575926532,0.8767742784,0.7642756841
112,0.7554318975,0.8776998072,0.7613852114
113,0.7557062886,0.8748985984,0.7628110334
114,0.762668324,0.8765257161,0.7652698975
115,0.7595411742,0.8773332063,0.766028636
116,0.7600455187,0.8777419864,0.7629296289
117,0.7593939411,0.8778207954,0.7627626259
118,0.7570133448,0.8746856184,0.7616273867
119,0.7581570186,0.8782609984,0.7646573867
120,0.7593956512,0.8781301039,0.7644490793
121,0.7614096846,0.8797955604,0.7647872083
122,0.7581675239,0.879778132,0.7662263872
123,0.7598524184,0.8787675352,0.7630569109
124,0.7567538178,0.878625262,0.7573535708
125,0.7588798937,0.8776751436,0.7610787197
126,0.7591554731,0.879048916,0.7647083611
127,0.7577864885,0.878428493,0.7648886983
128,0.7569162476,0.8785815864,0.76439843
129,0.7608949572,0.878551476,0.7631915037
130,0.7613248886,0.8795707575,0.7628964439
131,0.7599503935,0.8798563887,0.7643010985
132,0.7576835614,0.8771308393,0.7621426718
133,0.7606845284,0.8798921674,0.7670305535
134,0.7596403952,0.8805460957,0.7643238914
135,0.7627192622,0.8809933274,0.7645337216
136,0.7639349402,0.8809390656,0.7665093402
137,0.7588426364,0.8804600447,0.7635769684
138,0.7624129219,0.8819619098,0.7647672841
139,0.7595255838,0.8813936909,0.7670401474
140,0.7584254448,0.8811701567,0.7643603695
141,0.7651074858,0.8805329843,0.7661793058
142,0.7599588174,0.8795895813,0.7666266583
143,0.7625063244,0.881313962,0.7648048196
144,0.7617455824,0.8829308547,0.7690192189
145,0.7637119779,0.8819704477,0.7634227403
146,0.7582602138,0.8833316682,0.7656176224
147,0.763669499,0.8822097311,0.7626321515
148,0.7602476656,0.8820756525,0.7642195118
149,0.7629271231,0.8818247505,0.7659864109
150,0.7592984398,0.8836053388,0.7615707685
151,0.7625887197,0.8845052515,0.7660699762
152,0.7631318614,0.8844912739,0.7657221148
153,0.7622365415,0.8847553866,0.7666085656
154,0.7621711525,0.8837533784,0.7664496774
155,0.7614274964,0.8854591852,0.7666081335
156,0.7621878182,0.8854259927,0.7670685542
157,0.7620735576,0.8855680366,0.7667554668
158,0.7631971636,0.8860435028,0.7671208565
159,0.7624255218,0.8855259546,0.7659171743
160,0.7625813048,0.8857892945,0.7655141227
161,0.7619512256,0.885522197,0.7655684834
162,0.7621068733,0.8861201021,0.7659177183
163,0.7620271953,0.8859834669,0.7665456661
164,0.7629767335,0.8862974271,0.7660374664
165,0.7622744496,0.8864353738,0.7668511713
166,0.7631364919,0.8871925554,0.7663567239
167,0.7620068986,0.8861800642,0.7670009062
168,0.7619855455,0.8864850476,0.7668593035
169,0.7623970382,0.8865769106,0.7659343415
170,0.761887961,0.8865092851,0.7666645894
171,0.7632992526,0.8869414118,0.7664351462
172,0.7628946127,0.8869959836,0.7671792699
173,0.7627457204,0.8870169453,0.7652590563
174,0.7629540244,0.8874093638,0.7658331971
175,0.7624376839,0.8878617121,0.7672992573
176,0.7623793092,0.8871885527,0.766280542
177,0.7630391732,0.8879483562,0.7662319549
178,0.7623282671,0.88781839,0.7667732892
179,0.7626936192,0.8879966895,0.7669847249
180,0.7625593084,0.8877983105,0.7671465996
181,0.7617197814,0.8888226854,0.7663499638
182,0.7623545765,0.8872379941,0.7668247277
183,0.7618127537,0.8886614372,0.7663599341
184,0.7636848678,0.8886104654,0.7673971574
185,0.763953072,0.8885572053,0.7677720742
186,0.7624199601,0.8883532416,0.7674878961
187,0.7633191143,0.8878626279,0.7674353483
188,0.7633451873,0.8883590556,0.7666850621
189,0.7626140035,0.8885721556,0.7668693327
190,0.7629601314,0.8886920731,0.7661513704
191,0.7619949819,0.88842651,0.7659209691
192,0.7625008692,0.8894311297,0.7669516912
193,0.7617509025,0.8888283837,0.7667664491
194,0.7638000999,0.8898647021,0.7667975
195,0.7614242119,0.8891078702,0.766881744
196,0.7632576232,0.8900135687,0.767809148
197,0.7629090132,0.8902832344,0.7668680117
198,0.7645265869,0.8905042459,0.7662334182
199,0.7619319608,0.8911150636,0.7682148676
200,0.7630518764,0.8901049514,0.7677085233
201,0.7629845822,0.8900572923,0.7665253376
202,0.7633755142,0.8906440561,0.7662524902
203,0.7631522478,0.8906827492,0.7666477371
204,0.7626092167,0.8904039542,0.7667473895
205,0.7632445137,0.8906928751,0.765560255
206,0.7636509954,0.8912354507,0.766821047
207,0.7624566272,0.8911345082,0.7660777185
208,0.7625925829,0.8909334949,0.7656282015
209,0.7636179856,0.8910432692,0.7664073269
210,0.7626334089,0.8907691559,0.7670691536
211,0.7623521325,0.8910046432,0.7665589452
212,0.762459098,0.8914658954,0.7665563134
213,0.7626785365,0.8911585315,0.7665399268
214,0.7628499426,0.8912500148,0.7663524159
215,0.7624638752,0.8908029486,0.7656692272
216,0.7625333028,0.8915764473,0.766934023
217,0.7623106743,0.8917732662,0.7660212687
218,0.7631942211,0.8916821182,0.7671667242
219,0.7627680811,0.892027496,0.767393295
220,0.7625380889,0.8918069147,0.7664701256
221,0.7625701313,0.8922049787,0.7655784973
222,0.7635558178,0.8920850923,0.7663406646
223,0.762825007,0.8919986922,0.7669572692
224,0.7602514235,0.8923344447,0.7668637714
225,0.762387628,0.89197,0.7669498329
226,0.7618936323,0.8920659274,0.7674469168
227,0.762447557,0.8914806381,0.7669580119
228,0.7627006614,0.8926028185,0.7665798038
229,0.7627600819,0.892636341,0.7670402533
230,0.7624151832,0.8928519171,0.7674819812
231,0.7625499507,0.8933163754,0.7675158284
232,0.7617516661,0.8930002653,0.7669384916
233,0.7632137687,0.8928423599,0.7662246289
234,0.7615827435,0.8924830247,0.7660483215
235,0.7628534525,0.8929476213,0.7674084392
236,0.7645616831,0.8936801555,0.7678168203
237,0.7633341797,0.8932778935,0.7663613023
238,0.7630247959,0.8927369543,0.7676437569
239,0.7641403056,0.8934310902,0.767321626
240,0.7635309414,0.8932157619,0.7659339666
241,0.7634770989,0.8931823067,0.765858948
242,0.7639010899,0.893841582,0.7674870325
243,0.7621259052,0.893091128,0.7668048564
244,0.7639107991,0.8943769788,0.7666268379
245,0.7637940802,0.8937606805,0.7674824161
246,0.7630042537,0.8934404208,0.7671679787
247,0.7636537952,0.8933398535,0.7670220147
248,0.7618421085,0.8937845781,0.7675570355
249,0.7637221986,0.8944391888,0.7666045104
250,0.7631147693,0.8939187527,0.7683511487
251,0.7627357785,0.8940759873,0.7667456557
252,0.7632110865,0.8940665501,0.7677048202
253,0.7631554228,0.8948733918,0.7674493015
254,0.7635703288,0.8946539914,0.7669909877
255,0.7631356675,0.8948346125,0.7657909793
256,0.7639520112,0.8947924617,0.7672535065
257,0.7631942211,0.8953647396,0.7655636421
258,0.7619019781,0.8951113669,0.7676145602
259,0.763332221,0.8954967118,0.7666805142
260,0.763909908,0.895045003,0.7669269342
261,0.7637054729,0.895702937,0.7662545577
262,0.762767443,0.8949112811,0.7671528841
263,0.7625507766,0.8960739511,0.7672434347
264,0.7630566852,0.895474021,0.7672327069
265,0.7638642645,0.8954688067,0.7672239524
266,0.7632996578,0.895188046,0.7654795722
267,0.7630575388,0.8958213799,0.7671925028
268,0.7619832062,0.8955594372,0.7669165676
269,0.7642116647,0.8952875222,0.7661545999
270,0.763160537,0.8956355328,0.76651994
271,0.7631560307,0.8959218806,0.7672169598
272,0.7632254907,0.8963342137,0.7674233298
273,0.7631268773,0.8957156433,0.7663774065
274,0.7628022311,0.8966991537,0.7676553572
275,0.7639075831,0.8960580519,0.7667169355
276,0.7639521595,0.8962759972,0.7678824677
277,0.7634854056,0.8964377793,0.7670529657
278,0.7629619075,0.8966324767,0.7679443663
279,0.763390942,0.896645471,0.7669395953
280,0.7641281153,0.8966049026,0.7668292284
281,0.7644703727,0.896703745,0.7665631167
282,0.7638993185,0.8966853772,0.7679608094
283,0.7641748107,0.8966424519,0.7682697791
284,0.7635681679,0.8967858079,0.7673145143
285,0.7630418034,0.8962522237,0.7685723674
286,0.7627086807,0.8972982025,0.767068633
287,0.7642817099,0.8967366784,0.7670568
288,0.7628047949,0.8975354871,0.7664977749
289,0.7630747037,0.8969741402,0.7674801722
290,0.764433997,0.8969978808,0.7678824677
291,0.764265201,0.8968920788,0.7672705214
292,0.7624150393,0.8976466032,0.7670925526
293,0.7624104068,0.8978316798,0.768304348
294,0.763496451,0.8975280619,0.7681192057
295,0.7647727423,0.8979118372,0.7686131381
296,0.7635171438,0.8977131737,0.7673471906
297,0.7642340845,0.8978135298,0.7690564164
298,0.7639269847,0.8983843803,0.7685077829
299,0.7642740369,0.8980630302,0.7689137631
300,0.7632915522,0.8984475009,0.7684243086


==> csv/precision.tex <==
epochs,FINE,PASS,SmallLoss
50,0.5194046634,0.9660496189,0.6662237402
51,0.603371761,0.9659791363,0.6631665597
52,0.6303093129,0.965019786,0.6602885348
53,0.6477744329,0.9660508914,0.6635090087
54,0.640629032,0.9663595155,0.6629422523
55,0.6499121838,0.9665723605,0.6650405518
56,0.6515332451,0.9677021526,0.6650057819
57,0.6528050737,0.9668269186,0.6649792986
58,0.6486631009,0.9659266612,0.6648209966
59,0.6488077965,0.9669694846,0.6633102716
60,0.6512117384,0.9671413857,0.6628398435
61,0.6542020376,0.9676765386,0.6652360972
62,0.6516570358,0.9676369528,0.6646958978
63,0.6536853738,0.966857955,0.66279986
64,0.654100303,0.9657453916,0.6654717691
65,0.6508648077,0.9675215521,0.6634872663
66,0.6564396677,0.9677672878,0.6651346309
67,0.6536860819,0.9673595682,0.664756036
68,0.6568716787,0.9669170094,0.663147562
69,0.6561623413,0.9673501626,0.6655781439
70,0.656656377,0.9671572636,0.666540157
71,0.6551014135,0.9682975699,0.6683584128
72,0.6563899626,0.9673075856,0.6665531552
73,0.65732722,0.9675181252,0.6677445638
74,0.6589031046,0.9681721527,0.6651050371
75,0.6549130035,0.9673058073,0.6682374941
76,0.6591717121,0.9680490521,0.6639431567
77,0.658853592,0.9680932071,0.6685601691
78,0.6557501259,0.967314845,0.663396368
79,0.6592718306,0.9685220956,0.6687914447
80,0.6566996927,0.9675885151,0.6661252315
81,0.6567549396,0.9693768395,0.6692844961
82,0.6567498214,0.9686718631,0.6693683489
83,0.6572582947,0.9693717011,0.667051375
84,0.6587542461,0.9690003516,0.6673125214
85,0.6580406391,0.9693214913,0.6683483153
86,0.6567023841,0.9687320198,0.6674210584
87,0.6588770301,0.9688284548,0.6678550781
88,0.6592964686,0.9693416208,0.6687213771
89,0.6567820861,0.9694331816,0.6704183268
90,0.6615087611,0.9689456347,0.669686266
91,0.6593801504,0.9684292673,0.6679437382
92,0.6649650435,0.9684641227,0.6680133776
93,0.6549546571,0.9685211408,0.6701542911
94,0.6645667596,0.9680564068,0.6715219923
95,0.6609701185,0.968277015,0.668227187
96,0.6616322775,0.9685877971,0.6718769366
97,0.6650742277,0.9675365557,0.6708575732
98,0.6650239832,0.9681558083,0.6739340224
99,0.664041531,0.9683105571,0.6701828495
100,0.6628800778,0.9674641122,0.6729488476
101,0.665943747,0.96891552,0.6730739723
102,0.663587509,0.9688761078,0.6713837929
103,0.6687112676,0.9683793171,0.6727956919
104,0.6689302766,0.9674720454,0.6751033972
105,0.6676092664,0.9678998539,0.6747557105
106,0.6660268036,0.9681189983,0.6748189338
107,0.6676229036,0.9690679691,0.6699181151
108,0.6659381104,0.968707694,0.6761752787
109,0.663266822,0.9685586646,0.6736698481
110,0.668560877,0.9688673328,0.6707875488
111,0.6666985314,0.9685300709,0.6734341345
112,0.664905755,0.9694971094,0.6726896318
113,0.6656101642,0.9681855559,0.6718366851
114,0.6688501006,0.9679236599,0.6753784683
115,0.6690686352,0.9688374516,0.674779833
116,0.6673513652,0.9681362109,0.6729788658
117,0.6696807833,0.9689127802,0.6731883543
118,0.6661723418,0.9684918562,0.6703734751
119,0.666992982,0.9703970717,0.6744014864
120,0.6664873371,0.9690225644,0.6752290162
121,0.6706404172,0.9702133469,0.672346893
122,0.6662699758,0.9691228187,0.6738560818
123,0.6686215248,0.9696976077,0.6727085028
124,0.6672605696,0.9700534629,0.6685932285
125,0.6673479285,0.9694956284,0.6710835055
126,0.6675198986,0.9688064474,0.6734066866
127,0.6667900435,0.9684056332,0.6744802282
128,0.6657903598,0.9683698468,0.6740221296
129,0.6678350992,0.9688212849,0.6737625927
130,0.6698353851,0.96920088,0.676390642
131,0.6689357036,0.9682683424,0.674668432
132,0.664720398,0.9684612258,0.6731872676
133,0.6710560178,0.9685867845,0.6765705031
134,0.6691294267,0.968491735,0.6732991329
135,0.6729094584,0.9688803179,0.6741857056
136,0.674051055,0.97037112,0.67487387
137,0.6682875368,0.9692094456,0.6745052054
138,0.6724795877,0.9690296408,0.6737775929
139,0.6688349214,0.9690401609,0.6759538089
140,0.6681758871,0.9688460072,0.6740331709
141,0.6732356562,0.9688069655,0.6764663559
142,0.6689255396,0.9688395917,0.6765284218
143,0.6695161347,0.9686744375,0.6741393323
144,0.6719100145,0.9689536143,0.6800264622
145,0.6733292075,0.969165422,0.6740289022
146,0.6688777033,0.9695178386,0.6773870172
147,0.6726796444,0.9692250038,0.67305561
148,0.6694430123,0.9689013983,0.6748473158
149,0.6691112488,0.9695629031,0.6753211938
150,0.6680650359,0.9694892318,0.6719428708
151,0.6713059312,0.9691391797,0.6749139152
152,0.6707808221,0.9690486429,0.6747236608
153,0.6696284774,0.9688854985,0.6751207763
154,0.6700344689,0.9686447892,0.6738316808
155,0.6698552431,0.9691521875,0.6749340589
156,0.6700140689,0.9690159154,0.675578305
157,0.6695379715,0.9688456972,0.6740735077
158,0.670191186,0.9689641,0.6744998345
159,0.669506318,0.9685750396,0.6736552661
160,0.6696776862,0.9684127975,0.6736103567
161,0.6688210274,0.9683962361,0.6737641293
162,0.6694973545,0.9682995988,0.6742123932
163,0.66930541,0.9684248313,0.6734497937
164,0.6704259473,0.9678211482,0.6739108598
165,0.6691128331,0.9683192013,0.6736912681
166,0.6701205797,0.968099579,0.6741734498
167,0.6696192645,0.9679916673,0.6744298727
168,0.6693561047,0.9680997649,0.6748357267
169,0.6695772331,0.9681499943,0.6743775702
170,0.6693665334,0.9681012815,0.6744878804
171,0.6702108693,0.9679505771,0.6747820883
172,0.6703451983,0.9676876657,0.6747982649
173,0.6700923031,0.9683553271,0.6730072011
174,0.6703448294,0.968335236,0.6735022252
175,0.6699620423,0.9677867539,0.6748682327
176,0.6697798231,0.9679217125,0.6738242586
177,0.6701312542,0.9678808297,0.6742583261
178,0.6700234914,0.9677397159,0.6746098246
179,0.6702651627,0.9678838729,0.6739665336
180,0.6703574492,0.967915707,0.6748402882
181,0.6697523178,0.9678915984,0.6740703983
182,0.6703180354,0.967702992,0.6748053659
183,0.669711321,0.9684572373,0.6741321148
184,0.6710818657,0.9678339965,0.6747422497
185,0.6717732336,0.9678748863,0.6761343126
186,0.6701651692,0.968172104,0.6752991329
187,0.6705862213,0.9675653939,0.6757051636
188,0.6710643578,0.9679066784,0.6747978097
189,0.6703266111,0.9677431106,0.67489765
190,0.6704463775,0.9679718728,0.6742494703
191,0.6696699896,0.9679551954,0.674170992
192,0.6701748685,0.9676649294,0.6749788296
193,0.669569586,0.9676267189,0.6745066027
194,0.6711216186,0.9676923851,0.6750649441
195,0.6696418899,0.9677327788,0.6752187878
196,0.6706984839,0.9678782053,0.675634333
197,0.6704365474,0.9678510852,0.6750116423
198,0.6716447206,0.9680413276,0.6741447067
199,0.6694574825,0.9679914806,0.6764255762
200,0.6705880797,0.9679280673,0.6755016937
201,0.670853247,0.9677045727,0.6746663871
202,0.6713191487,0.9678738043,0.6747546361
203,0.6702827177,0.967744119,0.6749954574
204,0.6702961501,0.9676384081,0.6747551563
205,0.6706782386,0.9674367429,0.6737745841
206,0.6708684121,0.9677790216,0.6746605929
207,0.6698301402,0.9678166453,0.6745301282
208,0.6703165782,0.9672323938,0.6748813389
209,0.6713475296,0.9677668901,0.6748551991
210,0.6707030422,0.9678376367,0.6757655874
211,0.6701757143,0.9678964913,0.6749972894
212,0.6699720784,0.9678815043,0.6745519789
213,0.6706110415,0.9678181597,0.6745729798
214,0.670691277,0.9676480286,0.6745145177
215,0.6700024897,0.9677517129,0.6744550449
216,0.6705713199,0.9677565839,0.6751139382
217,0.6707360065,0.9677250833,0.6741175363
218,0.6704854767,0.9676753942,0.6754514085
219,0.6699198505,0.9678289674,0.6758725834
220,0.670601842,0.9676393835,0.6749991223
221,0.670489625,0.967752358,0.6741978695
222,0.6712052754,0.9677447863,0.6743803127
223,0.6707220123,0.9678710757,0.6751964258
224,0.6684290528,0.9676727937,0.6758432695
225,0.6697696534,0.9676936122,0.6749063681
226,0.6699749434,0.9676996803,0.676142185
227,0.6705311705,0.9675308495,0.6748958477
228,0.6701838843,0.9678651946,0.6754955853
229,0.6711305761,0.9675604192,0.6754645898
230,0.6701347219,0.9677931838,0.6758705104
231,0.6705508393,0.9679538788,0.6757137186
232,0.6701485937,0.9675397409,0.6749583827
233,0.6713002079,0.9678802651,0.6748277712
234,0.6697021489,0.967638351,0.6747172134
235,0.6706505264,0.9675801811,0.6759659414
236,0.6722984615,0.9681519061,0.6762269956
237,0.670931987,0.9676448999,0.6748768681
238,0.6707307206,0.9677420933,0.6760749075
239,0.671393631,0.9677859038,0.676040945
240,0.6707981481,0.9677723202,0.6740055127
241,0.6710836277,0.9678578221,0.6747728401
242,0.6715081343,0.9671128095,0.6759016153
243,0.6701261658,0.9673704932,0.6753554479
244,0.6715692982,0.9674961338,0.6744989347
245,0.6714581346,0.9674132203,0.6755690175
246,0.6705375659,0.9674802285,0.6753371733
247,0.6710108477,0.9672989474,0.6754130418
248,0.6704740741,0.9674147443,0.6753598356
249,0.6712547712,0.9675873778,0.6747890647
250,0.6705469785,0.9677291829,0.6761723071
251,0.6707226698,0.9673896652,0.6753567359
252,0.6711572989,0.9674763827,0.6761463594
253,0.6706788832,0.9675712956,0.6759129113
254,0.6712969473,0.9676009999,0.6760175514
255,0.6703031094,0.967263736,0.6742250397
256,0.672141817,0.9676534035,0.6753768261
257,0.6704854767,0.9676896076,0.6741050453
258,0.6699647399,0.9673685425,0.6757738208
259,0.6706064528,0.967132142,0.6749533107
260,0.6713142315,0.9675385932,0.675498283
261,0.6708374826,0.967667432,0.675013956
262,0.6703561495,0.9674429183,0.6752441205
263,0.6701136637,0.9675603781,0.6753147855
264,0.670618557,0.9675658299,0.6750662332
265,0.6711516155,0.9673913513,0.6753774711
266,0.6709017092,0.9675476772,0.673765622
267,0.6704355836,0.9674573298,0.6753055116
268,0.6692145627,0.9674406504,0.6747621387
269,0.6711587702,0.9672927254,0.6742080874
270,0.6702725236,0.9674019845,0.6744492889
271,0.6698066829,0.9676377546,0.6747871723
272,0.6701200885,0.9671425229,0.6755703428
273,0.6700598407,0.9671027563,0.6738123192
274,0.6696969947,0.9668625442,0.6757209169
275,0.6709884086,0.9670379439,0.6750562511
276,0.671517841,0.9667917735,0.6755393067
277,0.6706358534,0.9668456104,0.6748111381
278,0.6700809922,0.9668149036,0.6757973737
279,0.6703522603,0.9664694427,0.6753317455
280,0.6710069327,0.9670731668,0.6746500922
281,0.6717881673,0.9668195258,0.6746552976
282,0.6709986481,0.9669916471,0.6754753606
283,0.6714238829,0.9669455347,0.6759767439
284,0.6705337336,0.9671715223,0.6754481492
285,0.6702732346,0.9667902303,0.6756585002
286,0.6699201417,0.9670744612,0.6750903823
287,0.6714738241,0.9667350571,0.6744700933
288,0.6698386537,0.9670897294,0.674067776
289,0.6713628066,0.9667504906,0.6750093372
290,0.6718702689,0.9667520332,0.6755393067
291,0.6714943742,0.9663991309,0.6755425984
292,0.6698810198,0.9664917866,0.6748724172
293,0.6701042802,0.9665470576,0.676007094
294,0.6703313262,0.9664840264,0.6763237489
295,0.6720708464,0.9664659981,0.6772298702
296,0.6709610614,0.9665393122,0.6754059117
297,0.6714233178,0.9667185845,0.677102671
298,0.6711103479,0.9662815096,0.6763453413
299,0.670498565,0.9663896559,0.6768350948
300,0.6704746761,0.9665872755,0.6760769666

==> main/probability_agreement_graph.tex <==
\begin{figure}[t!]
    \centering
    \begin{tikzpicture}
        \pgfplotstableread[col sep=comma, header=true]{cosine_data.txt} \myTable
        \begin{axis}[
            height=0.37\linewidth,
            width=0.85\linewidth,
            xlabel={Number of epochs},
            xlabel style={font=\footnotesize},
            xticklabel style={font=\footnotesize},
            ylabel={Cosine similarity +/- std},
            ylabel style={font=\footnotesize, yshift=-0.5em},
            yticklabel style={font=\footnotesize},
            xmin=20,
            xmax=260,
            legend style={draw=none, font=\footnotesize, yshift=-2em, /tikz/every even column/.append style={column sep=1em}},
            legend columns=2,
            scale only axis
        ]
            \addlegendentry{clean};
            \addplot[mark=*, mark size=1.5pt, mark repeat=0, mark phase=0, MidnightBlue!70, thick, solid] plot [error bars/.cd, y dir=both, y explicit] table[x={epochs}, y={cleanCosine}, y error={cleanStd}]{\myTable};

            \addlegendentry{noisy};
            \addplot[mark=diamond*, mark size=1.5pt, BurntOrange!70, thick, solid] plot [error bars/.cd, y dir=both, y explicit] table[x={epochs}, y={noisyCosine}, y error={noisyStd}]{\myTable};
            
            % \addplot[MidnightBlue!40, opacity=0.4] table[x={epochs}, y expr=\thisrow{cleanCosine}-\thisrow{cleanStd}]{\myTable};
            % \addplot[BurntOrange!40, opacity=0.4] table[x={epochs}, y expr=\thisrow{noisyCosine}-\thisrow{noisyStd}]{\myTable};
            
            % \addplot[MidnightBlue!40, opacity=0.4] table[x={epochs}, y expr=\thisrow{cleanCosine}+\thisrow{cleanStd}]{\myTable};
            % \addplot[BurntOrange!40, opacity=0.4] table[x={epochs}, y expr=\thisrow{noisyCosine}+\thisrow{noisyStd}]{\myTable};
        \end{axis}
    \end{tikzpicture}
    % \vspace{-2.5em}
    \caption{Probability agreement of clean- and noisy-label samples on CIFAR100~\cite{krizhevsky2009learning} at \(0.5\) IDN~\cite{xia2020part} using DivideMix-PASS. It shows the cosine similarity with standard deviation between clean samples (\textcolor{MidnightBlue}{blue}) and the cosine similarity with standard deviation between noisy samples (\textcolor{BurntOrange}{orange}) over the number of epochs. }
    \label{fig:cosinehypothesis}
\end{figure}

==> main/train_loss_dm_pass.tex <==
\begin{figure}[t!]
    \centering
    \begin{tikzpicture}
        \pgfplotstableread[col sep=comma, header=true]{smoothed_loss_data.txt} \myTable
        \begin{axis}[
            height=0.37\linewidth,
            width=0.85\linewidth,
            xlabel={Number of epochs},
            xlabel style={font=\footnotesize},
            xticklabel style={font=\footnotesize},
            ylabel={Loss Values},
            ylabel style={font=\footnotesize, yshift=-0.5em},
            yticklabel style={font=\footnotesize},
            xmin=30, xmax=302, % Adjust x-axis limits as per your data
            legend style={draw=none, font=\footnotesize, yshift=-2em, /tikz/every even column/.append style={column sep=1em}},
            legend columns=2,
            scale only axis
        ]
            \addlegendentry{DivideMix-PASS (Ours)};
            \addplot[mark=*, mark size=1.5pt, mark repeat=0, mark phase=0, MidnightBlue!70, thick, solid] table[x={Epoch}, y={TotalLoss}]{\myTable};

            % \addlegendentry{Labeled Loss (Your Approach)};
            % \addplot[mark=square*, mark size=1.5pt, BurntOrange!70, thick, solid] table[x={Epoch}, y={LabeledLoss}]{\myTable};
            
            \addlegendentry{DivideMix};
            \addplot[mark=square, mark size=1.5pt, ForestGreen!70, thick, solid] table[x={Epoch}, y={DM_TotalLoss}]{\myTable};

            % \addlegendentry{DM Labeled Loss};
            % \addplot[mark=triangle*, mark size=1.5pt, Red!70, thick, solid] table[x={Epoch}, y={DM_UnlabeledLoss}]{\myTable};
        \end{axis}
    \end{tikzpicture}
    \caption{Comparison of training loss over epochs between DivideMix-PASS (ours) and DivideMix~\cite{li2020dividemix} on CIFAR-100~\cite{krizhevsky2009learning} at \(0.5\) IDN~\cite{xia2020part}. 
    \gustavo{Why do we need this figure?}
    %\textcolor{MidnightBlue}{\textbf{--}} represents DivideMix-PASS, \textcolor{ForestGreen}{\textbf{- -}} indicates DivideMix~\cite{li2020dividemix}.
    }
    \label{fig:lossComparison}
\end{figure}

==> supp_cifar0.2_csv/clean.tex <==
0,epochs,FINE,SmallLoss,PASS
0,50,0.82704,0.66028,0.6923767999999999
1,51,0.69504,0.65618,0.6951144
2,52,0.70858,0.66386,0.6918812
3,53,0.70572,0.65832,0.6948076
4,54,0.69542,0.6461,0.6959875999999999
5,55,0.6859,0.64358,0.6898752
6,56,0.69064,0.64812,0.6905595999999999
7,57,0.67958,0.64162,0.6931791999999999
8,58,0.67728,0.64298,0.6945716
9,59,0.67264,0.64678,0.6962944
10,60,0.67086,0.64492,0.6962235999999999
11,61,0.67012,0.64104,0.693958
12,62,0.66898,0.65008,0.6951379999999999
13,63,0.6683,0.6421,0.6955627999999999
14,64,0.66254,0.64736,0.6961999999999999
15,65,0.66874,0.63972,0.6975452
16,66,0.66376,0.63784,0.6951144
17,67,0.6655,0.65054,0.6973328
18,68,0.6667,0.64544,0.6949963999999998
19,69,0.66344,0.64426,0.696554
20,70,0.65356,0.64936,0.6959167999999999
21,71,0.66516,0.64258,0.6979464
22,72,0.66778,0.64464,0.6984892
23,73,0.6661,0.64784,0.6992916
24,74,0.66184,0.64206,0.6965068
25,75,0.66104,0.64058,0.6968371999999999
26,76,0.65738,0.63962,0.6996928
27,77,0.64608,0.64666,0.6992444
28,78,0.65854,0.64868,0.7020292
29,79,0.65828,0.64454,0.6998816
30,80,0.65406,0.63854,0.6999759999999999
31,81,0.66012,0.63914,0.6967428
32,82,0.6564,0.63704,0.7049791999999999
33,83,0.65932,0.6425,0.7033744000000001
34,84,0.6505,0.63636,0.7033744000000001
35,85,0.65022,0.6385,0.7034216
36,86,0.6494,0.63664,0.7034216
37,87,0.64816,0.6472,0.7041532
38,88,0.6489,0.64506,0.7063008
39,89,0.65084,0.64662,0.7040351999999999
40,90,0.64932,0.64768,0.7028316
41,91,0.64962,0.64696,0.7060175999999999
42,92,0.64656,0.64476,0.7072448
43,93,0.6546,0.64608,0.7078819999999999
44,94,0.6473,0.6476,0.7069616
45,95,0.6596,0.64848,0.7077167999999999
46,96,0.64822,0.6468,0.7086372
47,97,0.65274,0.64106,0.7059232
48,98,0.65408,0.64258,0.7084955999999999
49,99,0.65286,0.64204,0.7060647999999999
50,100,0.64916,0.65176,0.70446
51,101,0.65506,0.64326,0.712602
52,102,0.6482,0.64578,0.7084484
53,103,0.64848,0.6579,0.7100296
54,104,0.6472,0.6455,0.71213
55,105,0.6548,0.64348,0.7111152
56,106,0.65796,0.64904,0.7096284
57,107,0.65548,0.65088,0.7082596
58,108,0.65176,0.64436,0.7113512
59,109,0.65316,0.6478,0.7119648
60,110,0.6494,0.6507,0.7112567999999999
61,111,0.65334,0.64578,0.7132628
62,112,0.64898,0.65474,0.7120591999999999
63,113,0.65718,0.65074,0.7129088
64,114,0.65412,0.6491,0.7139
65,115,0.65278,0.65066,0.7173692
66,116,0.65354,0.64978,0.7119411999999999
67,117,0.65324,0.64926,0.7173927999999999
68,118,0.65494,0.64952,0.7165431999999999
69,119,0.65242,0.64516,0.7170388
70,120,0.65608,0.65162,0.7111152
71,121,0.6524,0.64616,0.7164724
72,122,0.65242,0.662,0.716024
73,123,0.65384,0.6483,0.7162599999999999
74,124,0.65272,0.64996,0.7177232
75,125,0.65386,0.64904,0.7181951999999999
76,126,0.65648,0.6512,0.717204
77,127,0.6504,0.65302,0.717086
78,128,0.65934,0.64836,0.7172276
79,129,0.65414,0.65514,0.7189739999999999
80,130,0.65588,0.65412,0.7159531999999998
81,131,0.65866,0.653,0.719446
82,132,0.65412,0.6478,0.7163544
83,133,0.6548,0.64876,0.7175579999999999
84,134,0.65276,0.64468,0.720154
85,135,0.6568,0.64768,0.7198943999999999
86,136,0.6561,0.65194,0.7198708
87,137,0.64776,0.65766,0.71744
88,138,0.65108,0.65252,0.7204844
89,139,0.6565,0.66488,0.7200123999999999
90,140,0.65376,0.64614,0.7207439999999999
91,141,0.66368,0.65108,0.7198236
92,142,0.65888,0.66296,0.7194223999999999
93,143,0.6533,0.6532,0.7204844
94,144,0.65552,0.66574,0.7204135999999999
95,145,0.65414,0.6549,0.7229388
96,146,0.65178,0.6586,0.7229151999999999
97,147,0.6566,0.65458,0.7212632
98,148,0.66472,0.65842,0.7250392
99,149,0.65708,0.65612,0.7239535999999999
100,150,0.65814,0.66042,0.7216408
101,151,0.66582,0.66436,0.7272339999999999
102,152,0.6671,0.66262,0.7299244
103,153,0.66856,0.66576,0.730302
104,154,0.66818,0.66956,0.7318832
105,155,0.66914,0.66636,0.7314584
106,156,0.67176,0.67014,0.732426
107,157,0.6717,0.6698,0.7326147999999999
108,158,0.67062,0.67096,0.7336531999999999
109,159,0.67112,0.67236,0.7345028
110,160,0.67252,0.6717,0.73632
111,161,0.67354,0.67356,0.7351872
112,162,0.67484,0.67372,0.7365796
113,163,0.6743,0.67662,0.7365796
114,164,0.67476,0.67426,0.7371931999999999
115,165,0.67596,0.67548,0.737264
116,166,0.67598,0.67518,0.7383968
117,167,0.6773,0.6752,0.7370515999999999
118,168,0.67836,0.6762,0.7388688
119,169,0.67786,0.67746,0.7390576
120,170,0.67866,0.67736,0.7394352
121,171,0.67882,0.67754,0.7403084
122,172,0.6798,0.67904,0.740686
123,173,0.67856,0.6796,0.7409927999999999
124,174,0.67916,0.67904,0.7402612
125,175,0.68006,0.67966,0.739742
126,176,0.68134,0.68068,0.7429044
127,177,0.67996,0.68254,0.7412288
128,178,0.68256,0.68012,0.7412523999999999
129,179,0.68262,0.6807,0.7425976
130,180,0.6818,0.68104,0.7431403999999999
131,181,0.68116,0.68254,0.7438719999999999
132,182,0.68248,0.6822,0.7437539999999999
133,183,0.68372,0.68224,0.7434236
134,184,0.68356,0.68288,0.7443676
135,185,0.68292,0.68414,0.7444147999999999
136,186,0.68396,0.68296,0.7459015999999999
137,187,0.68422,0.68368,0.7454531999999999
138,188,0.68502,0.68374,0.7445327999999999
139,189,0.68542,0.68436,0.7464444
140,190,0.68602,0.68502,0.7461376
141,191,0.68498,0.68512,0.7461848
142,192,0.68584,0.68506,0.7468691999999999
143,193,0.68632,0.68648,0.7474356
144,194,0.68742,0.68524,0.7466567999999999
145,195,0.68642,0.68616,0.746822
146,196,0.68822,0.68612,0.7473648
147,197,0.68816,0.68596,0.748002
148,198,0.68702,0.68738,0.7485919999999999
149,199,0.68858,0.68812,0.750244
150,200,0.68714,0.6878,0.748474
151,201,0.6878,0.68808,0.7509992
152,202,0.68886,0.68888,0.749536
153,203,0.68876,0.68802,0.750598
154,204,0.68748,0.68894,0.750244
155,205,0.68904,0.6888,0.7509048
156,206,0.68978,0.68912,0.7512588
157,207,0.69038,0.68942,0.750126
158,208,0.69014,0.68912,0.7520376
159,209,0.68978,0.69028,0.7521319999999999
160,210,0.69106,0.69106,0.752486
161,211,0.69186,0.6903,0.7520376
162,212,0.69086,0.69044,0.7511407999999999
163,213,0.69064,0.69062,0.7533828
164,214,0.6906,0.6907,0.7534772
165,215,0.69334,0.69174,0.7539256
166,216,0.69176,0.69128,0.7546335999999999
167,217,0.69198,0.69138,0.7539963999999999
168,218,0.6918,0.6926,0.7546099999999999
169,219,0.6912,0.69178,0.7547752
170,220,0.6916,0.6922,0.7551292
171,221,0.69202,0.69292,0.7560731999999999
172,222,0.6914,0.69262,0.75579
173,223,0.69288,0.69306,0.7556012
174,224,0.69308,0.69328,0.7561912
175,225,0.69264,0.69232,0.7572296
176,226,0.69324,0.69416,0.7558372
177,227,0.69318,0.69424,0.7570408
178,228,0.69318,0.69332,0.7561675999999999
179,229,0.69296,0.69318,0.756498
180,230,0.69432,0.69364,0.756616
181,231,0.69406,0.6947,0.7566632
182,232,0.69416,0.69436,0.7574891999999999
183,233,0.6944,0.69458,0.7585275999999999
184,234,0.69466,0.69514,0.7580319999999999
185,235,0.69468,0.6948,0.7580319999999999
186,236,0.69462,0.69416,0.75874
187,237,0.69454,0.6943,0.7584803999999999
188,238,0.69638,0.69534,0.7596132
189,239,0.69534,0.69488,0.7587636
190,240,0.69596,0.69502,0.7598256
191,241,0.69482,0.69658,0.7603683999999999
192,242,0.69596,0.69704,0.7599671999999998
193,243,0.69574,0.6958,0.7589288
194,244,0.69678,0.69546,0.7600616
195,245,0.697,0.6961,0.759802
196,246,0.69734,0.69658,0.7597548
197,247,0.69682,0.6964,0.7606515999999999
198,248,0.69686,0.69538,0.7615719999999999
199,249,0.6973,0.69618,0.7626812
200,250,0.69658,0.6961,0.7610528
201,251,0.6983,0.6962,0.7613832
202,252,0.69756,0.69804,0.7608404
203,253,0.69842,0.69712,0.7617608
204,254,0.69806,0.69698,0.7633891999999999
205,255,0.69938,0.6964,0.7626103999999999
206,256,0.6982,0.69668,0.7624924
207,257,0.69872,0.69724,0.7624216
208,258,0.69818,0.69698,0.76346
209,259,0.6979,0.69718,0.7638376
210,260,0.69888,0.69708,0.7629644
211,261,0.69998,0.69814,0.7636252
212,262,0.69942,0.69792,0.762398
213,263,0.69978,0.69792,0.7643568
214,264,0.70018,0.6977,0.7639083999999999
215,265,0.70032,0.69894,0.76464
216,266,0.69966,0.69898,0.7638848
217,267,0.7005,0.6988,0.765584
218,268,0.7007,0.69844,0.765466
219,269,0.70112,0.69884,0.76464
220,270,0.70064,0.6992,0.7663156
221,271,0.7013,0.69978,0.7649703999999999
222,272,0.70044,0.69888,0.7656312
223,273,0.70102,0.69814,0.766056
224,274,0.70146,0.69876,0.766056
225,275,0.70104,0.69952,0.763342
226,276,0.7014,0.69976,0.7661032
227,277,0.70178,0.69976,0.7659852
228,278,0.70078,0.7002,0.7673776
229,279,0.70194,0.70028,0.767944
230,280,0.70108,0.7008,0.7671652
231,281,0.70192,0.69954,0.7679675999999999
232,282,0.70286,0.70066,0.7671887999999999
233,283,0.70252,0.70088,0.7678731999999999
234,284,0.70326,0.70148,0.7678259999999999
235,285,0.70282,0.70172,0.7672595999999999
236,286,0.7027,0.70072,0.7627283999999999
237,287,0.70326,0.7011,0.7680856
238,288,0.70254,0.7017,0.7686519999999999
239,289,0.70356,0.70172,0.7683452000000001
240,290,0.70252,0.70184,0.7683452000000001
241,291,0.70324,0.70168,0.7695487999999999
242,292,0.70316,0.7021,0.7695723999999999
243,293,0.70336,0.70146,0.770304
244,294,0.7031,0.70246,0.7688408
245,295,0.70328,0.70248,0.7687228
246,296,0.70356,0.70306,0.769124
247,297,0.70366,0.70248,0.7691711999999999
248,298,0.70396,0.70236,0.7701388
249,299,0.7045,0.7031,0.7685103999999999
250,300,0.7053,0.70346,0.7705636

==> supp_cifar0.2_csv/f1.tex <==
epochs,FINE,PASS,SmallLoss
50,0.681930527,0.8995733544,0.847718029
51,0.8244583355,0.8982934991,0.8496482098
52,0.8795803188,0.9006404418,0.847367907
53,0.890388255,0.8970344955,0.8495599929
54,0.9067631008,0.890739692,0.8505180341
55,0.9046564159,0.8886146751,0.8459485705
56,0.9097544034,0.8915969238,0.8468808098
57,0.909370361,0.8874180004,0.8483483434
58,0.9073696685,0.888529619,0.8495855037
59,0.9071055635,0.8925179051,0.8506698162
60,0.9070929351,0.8897709274,0.8504922967
61,0.9062321123,0.8884176018,0.8488975575
62,0.9053223344,0.8942238372,0.8501760195
63,0.9058135694,0.889550477,0.850283182
64,0.9026334911,0.8919566059,0.8509229493
65,0.9056422373,0.8872713576,0.8514843845
66,0.9038605312,0.8869502281,0.8496482098
67,0.9045993346,0.8947001894,0.8513991784
68,0.9066828664,0.8923715181,0.8498846123
69,0.9042466432,0.8905838521,0.8512356194
70,0.8972357436,0.894616755,0.8505960475
71,0.905157981,0.8895425487,0.8518935988
72,0.9077377813,0.8900584071,0.8522103339
73,0.9039860845,0.890818341,0.8527725035
74,0.9024209834,0.8880719,0.8511385484
75,0.9030100622,0.8876843851,0.8512428448
76,0.899877062,0.8854948195,0.8531172327
77,0.8915282986,0.8916087872,0.8527394499
78,0.9011285547,0.893280453,0.8547501835
79,0.9004936169,0.8888509533,0.8533132155
80,0.8976151623,0.8862316919,0.8533154141
81,0.9019423599,0.886192655,0.8510487626
82,0.8996383421,0.8861401873,0.8569329684
83,0.9019044047,0.8904890053,0.8558159015
84,0.8956620793,0.8854226976,0.8558797303
85,0.8945688933,0.8872724884,0.8560402883
86,0.8950117569,0.8847573565,0.8557849645
87,0.8931213171,0.8925252312,0.8563582801
88,0.8946929011,0.8915761356,0.857723688
89,0.8962355361,0.8927098319,0.8564037838
90,0.8953281839,0.8918876562,0.8554375757
91,0.8956829793,0.8922785567,0.8573356857
92,0.8930916127,0.8908423059,0.8585062959
93,0.8988408798,0.8929883716,0.8587566991
94,0.8932807277,0.8922659631,0.8581822991
95,0.9018644059,0.8946994503,0.8588335275
96,0.8947397687,0.8925332278,0.859534864
97,0.8973038148,0.8890001634,0.8576528508
98,0.8992638262,0.8896055168,0.8592455137
99,0.8973949844,0.890575982,0.8574960236
100,0.8954578162,0.8943123674,0.8568271051
101,0.8988753695,0.8902551762,0.8626556258
102,0.8944097181,0.8923805137,0.8592765948
103,0.8952533393,0.9007841812,0.860434254
104,0.8928896397,0.8916621966,0.8617566291
105,0.8994322658,0.8916218101,0.8609928539
106,0.9017580748,0.8955048791,0.8600931403
107,0.8998843088,0.8967191275,0.8590820712
108,0.8974390546,0.8918571489,0.8614106862
109,0.8983142615,0.8938019917,0.8620251798
110,0.8957669058,0.8970226006,0.8614092959
111,0.8982622834,0.8924434693,0.862791949
112,0.8946281902,0.8998396693,0.8617715449
113,0.9007298541,0.8969901133,0.8626756806
114,0.899105505,0.8962435297,0.8632941717
115,0.8970200969,0.897118057,0.8656118742
116,0.8982255088,0.8955661341,0.8620089078
117,0.8975579422,0.8956098667,0.8654369936
118,0.8992869517,0.8953677672,0.8647910176
119,0.8975006169,0.8925976008,0.8650670972
120,0.9004638937,0.8975970251,0.8614390926
121,0.8979885655,0.8908485194,0.8648061468
122,0.8979408538,0.9044960296,0.8643075135
123,0.8988931669,0.8938069697,0.8649789642
124,0.8976028554,0.8960180214,0.8655996121
125,0.8986568602,0.8958197374,0.8661774119
126,0.9007034547,0.8965224957,0.865498699
127,0.8964036019,0.8982836331,0.8652904696
128,0.9027351909,0.8949224987,0.8655785626
129,0.8989320655,0.900331241,0.8666464464
130,0.900878411,0.8993698157,0.8647047752
131,0.9020346684,0.8991493367,0.8667780937
132,0.8996715843,0.8949352891,0.864916298
133,0.9001239306,0.8948504423,0.8656775041
134,0.8986396254,0.8921660175,0.8673889819
135,0.9008196141,0.8949065253,0.8673390325
136,0.9011705425,0.8979033418,0.8671955983
137,0.8948289614,0.9023614205,0.8652783273
138,0.8974881092,0.8981554341,0.8679328109
139,0.901032774,0.9069657175,0.8671650051
140,0.898706733,0.8934753391,0.867728011
141,0.905553933,0.8977527473,0.867036064
142,0.9030797176,0.9058430266,0.8667619667
143,0.8985463153,0.8984203002,0.8675508685
144,0.9004174338,0.9077959873,0.8675025473
145,0.8993093166,0.8997093753,0.8693506994
146,0.8981466533,0.9026302373,0.8694619029
147,0.9012340519,0.9004734258,0.8682094066
148,0.9068960498,0.9021177399,0.8706508912
149,0.9012823903,0.9003184602,0.8699771742
150,0.9026477953,0.9045652912,0.8684668004
151,0.9082819654,0.90758108,0.8723929504
152,0.9095497715,0.9063417688,0.8740205201
153,0.9103223175,0.9085637519,0.8743387967
154,0.9099770944,0.9112032497,0.8754042236
155,0.9108786475,0.9089484384,0.8748640945
156,0.9127582422,0.9115081975,0.8756424666
157,0.9126511733,0.9113186612,0.876087086
158,0.9117259417,0.9120533557,0.8765309688
159,0.9122844266,0.9133401782,0.876910942
160,0.9133203623,0.9129146417,0.8779388014
161,0.9140112333,0.9141640698,0.8773700612
162,0.9146570568,0.9140316432,0.8782395189
163,0.9143215336,0.9163556505,0.8783029735
164,0.9147859055,0.9146179276,0.8787770483
165,0.9157948362,0.9153917242,0.8788878648
166,0.9155591751,0.9152333943,0.8793913093
167,0.9165296299,0.9153107389,0.8788727116
168,0.9173076779,0.9159216089,0.8798333791
169,0.9167531602,0.9170354061,0.8800862816
170,0.9173400579,0.9166490829,0.8802748201
171,0.9174573611,0.9166561535,0.8806668401
172,0.917987761,0.9178190372,0.8808550543
173,0.9175794608,0.9181667264,0.8811862069
174,0.9177065461,0.9178190372,0.8808256226
175,0.9183030894,0.9182106606,0.8804160423
176,0.9193015396,0.9188944883,0.8827747547
177,0.9182924113,0.9199404984,0.8814701595
178,0.9198797721,0.9185473704,0.8812956614
179,0.9202358609,0.9188466105,0.8821905121
180,0.919762484,0.9190326705,0.882614564
181,0.9190450356,0.920127883,0.8831636887
182,0.9200088001,0.9198798294,0.8828952609
183,0.9210375036,0.9200339736,0.8826759038
184,0.9207960573,0.9205007602,0.8834291318
185,0.9205795639,0.9214810263,0.8834604376
186,0.9210248968,0.9206840347,0.8845090244
187,0.9210892816,0.9210212164,0.8838953465
188,0.9214215733,0.9208775624,0.8834753328
189,0.9220243561,0.9214537645,0.8848049289
190,0.9226473985,0.9219337746,0.8845385559
191,0.9220791842,0.9220064661,0.8845064583
192,0.9222670375,0.9215259378,0.8849592582
193,0.9226155086,0.922806881,0.8852070781
194,0.9232884782,0.9219688314,0.8850087874
195,0.9226256815,0.9225746461,0.8849913735
196,0.9238055649,0.92235842,0.8854135735
197,0.9238244897,0.9222422519,0.8856446002
198,0.9229985199,0.9235218935,0.8860974393
199,0.9241908365,0.9241202756,0.8873132563
200,0.9230855238,0.9238885621,0.8861461861
201,0.923563794,0.9239041816,0.8875573351
202,0.9242686839,0.9244207368,0.8868467218
203,0.9241963479,0.9238607381,0.8875463769
204,0.9232695862,0.924339432,0.8872499585
205,0.9243988644,0.924425231,0.8874952044
206,0.9248713848,0.9247813691,0.8880445656
207,0.9249931093,0.9248735083,0.8871722286
208,0.9251313975,0.9245942925,0.8882403148
209,0.9249960593,0.9254323563,0.8883656238
210,0.9257953034,0.9259951479,0.8889145993
211,0.9261850592,0.9253221339,0.8883668449
212,0.925526421,0.9254855183,0.8879669317
213,0.9256169677,0.9256777482,0.8893135954
214,0.925463453,0.9256731444,0.8892490333
215,0.9271880166,0.926485306,0.8896064376
216,0.9263622067,0.9262161008,0.8901970641
217,0.9262092229,0.9260389291,0.8897793747
218,0.9263910259,0.9269176863,0.8900551075
219,0.9258962606,0.9262649075,0.8902265945
220,0.925997707,0.9267543244,0.8903320032
221,0.9263003204,0.927147942,0.8910763447
222,0.9259781453,0.9269943702,0.8910175313
223,0.9269194255,0.9273109315,0.8907042628
224,0.9270633011,0.9273445857,0.8913432375
225,0.9269335778,0.926653842,0.8917690854
226,0.9271161073,0.927976987,0.8908587117
227,0.9273843419,0.928034441,0.8918353959
228,0.9271352245,0.9273733474,0.8911380939
229,0.9271015358,0.927334952,0.8913541621
230,0.9281412518,0.927416602,0.8915577659
231,0.9277054794,0.9281779442,0.8913357289
232,0.9279640846,0.9282451362,0.8920018619
233,0.9281364279,0.928278552,0.8927427975
234,0.9283230707,0.9286181304,0.892356234
235,0.9280884313,0.928311953,0.8925458788
236,0.9281698525,0.927976987,0.8930077386
237,0.9278634618,0.9279530192,0.8926488053
238,0.9294316911,0.9286370994,0.8932608759
239,0.9286241819,0.9283693601,0.8928967091
240,0.9291308405,0.9284075709,0.8936519765
241,0.928251149,0.9295255941,0.8938158124
242,0.9288819578,0.9295438541,0.8935546222
243,0.9288487275,0.9291535653,0.8928780273
244,0.929344833,0.9288476128,0.8936160898
245,0.9296266718,0.9291818355,0.8936366067
246,0.9299321053,0.9294633843,0.893605866
247,0.9294978531,0.9295833758,0.8941264629
248,0.9296508883,0.9288524926,0.8944723295
249,0.9298413007,0.9291147178,0.8953190961
250,0.929512675,0.9291196189,0.8945137998
251,0.9302452798,0.9291912549,0.8946022584
252,0.9303382438,0.9306320312,0.8941861101
253,0.9305174796,0.9299120587,0.8947845027
254,0.9303846423,0.929811891,0.8957784685
255,0.9314513648,0.9294589275,0.8953362906
256,0.9304224946,0.9295971826,0.8951965322
257,0.9309182183,0.9299979018,0.8951505638
258,0.9307191385,0.929749687,0.8958243847
259,0.9303946769,0.9298927809,0.8960060731
260,0.9309080938,0.9298212387,0.8956291933
261,0.9316926891,0.9307034788,0.8960577949
262,0.9314177262,0.9304840863,0.8951352401
263,0.9314879716,0.9304218957,0.8965319304
264,0.9318973675,0.9303268397,0.8961782367
265,0.9319349674,0.9310260215,0.8967784968
266,0.9315888785,0.9311167355,0.8959735406
267,0.9318767848,0.9309260911,0.8972632167
268,0.9322677601,0.9307312149,0.8972500045
269,0.9323803451,0.9310168124,0.8965890933
270,0.9321628938,0.931211557,0.8975469559
271,0.9325084341,0.9317495256,0.8967399013
272,0.9319583112,0.9309831965,0.8972937486
273,0.9324955663,0.9303925656,0.8976315782
274,0.9328086412,0.9308975361,0.8975053467
275,0.9322612849,0.9313776667,0.8957478555
276,0.9326417028,0.9314245176,0.8975358623
277,0.9327256365,0.9315488034,0.8975226842
278,0.9322004458,0.9319867038,0.8982960516
279,0.9327772998,0.9319815542,0.8985984853
280,0.9322897554,0.932165507,0.8982220164
281,0.9328872849,0.9315784037,0.8988660652
282,0.9334309791,0.9323143571,0.8984265701
283,0.9331274087,0.9324088512,0.8986789781
284,0.9338391037,0.9327736811,0.8987116187
285,0.9334025749,0.9328822539,0.8984091703
286,0.9335036334,0.9321085443,0.8954128842
287,0.9337770183,0.9324411843,0.8988159927
288,0.9333899902,0.9324333419,0.8991811984
289,0.9341140506,0.932944371,0.8987941779
290,0.9331894953,0.9329675801,0.8990464957
291,0.9336386672,0.9329780489,0.8995697564
292,0.933768131,0.9329040073,0.8996480107
293,0.9337238293,0.9324488974,0.9002449994
294,0.9337255429,0.9332840161,0.8993028798
295,0.9339153868,0.9331740453,0.8992268321
296,0.9340519648,0.9347721962,0.8993592106
297,0.9340608201,0.9344224229,0.8994526852
298,0.9343356475,0.9350887849,0.9000125944
299,0.9345942495,0.9356764187,0.8990268397
300,0.9350987316,0.9366215828,0.9004119813


==> supp_cifar0.2_csv/precision.tex <==
epochs,FINE,SmallLoss,PASS
50,0.5621674264,0.9843160342,0.9954196038
51,0.8205334009,0.9875531982,0.995437582
52,0.8938009399,0.9814581573,0.995416334
53,0.9142170875,0.982329343,0.9956955673
54,0.9529481823,0.9875949055,0.9959624972
55,0.9606296714,0.9871943472,0.9954030511
56,0.963738492,0.9863507393,0.996323573
57,0.9767125,0.9877448534,0.9955551752
58,0.9760857065,0.987888208,0.9960844191
59,0.9815832537,0.9899506792,0.9958344876
60,0.9838855914,0.9874551583,0.9955745476
61,0.983307002,0.9904535456,0.9955601471
62,0.9831665768,0.9884851415,0.99647782
63,0.9849510223,0.9910609269,0.9960899828
64,0.9868713134,0.9880863322,0.9964831788
65,0.9840601052,0.9901965724,0.9957124069
66,0.9874646467,0.992313874,0.995437582
67,0.986475108,0.9887260866,0.9958406714
68,0.9886548035,0.9915782222,0.9960868055
69,0.9885995263,0.9899116652,0.9966148218
70,0.9892403169,0.990224128,0.9962218694
71,0.9879457427,0.9903580663,0.9959737948
72,0.9891269704,0.9883888051,0.9958475363
73,0.984562657,0.9852969854,0.9958522864
74,0.9874286201,0.9883425504,0.9964847239
75,0.9895906068,0.9897356893,0.9962268457
76,0.9888410732,0.9869976719,0.9959838141
77,0.9891167504,0.9884247647,0.9958520073
78,0.9895513955,0.9886940308,0.9959971406
79,0.9887410903,0.9862756969,0.9961140412
80,0.9892484768,0.9899408252,0.9959854342
81,0.9888870101,0.9890008687,0.9959668604
82,0.9897487695,0.9919456909,0.9962703026
83,0.9899089398,0.9922507604,0.9962618166
84,0.99059027,0.991578363,0.9963903749
85,0.988952315,0.9919639984,0.9966477897
86,0.9909255259,0.9899110287,0.9961335414
87,0.9891513951,0.9893710454,0.9962659396
88,0.9910357384,0.9906303905,0.996021278
89,0.9911791154,0.9905353493,0.9965222167
90,0.9916272196,0.987508122,0.9962589375
91,0.9918653871,0.9892499309,0.9956357399
92,0.9913563632,0.9896840519,0.9962822175
93,0.9907648892,0.9918220774,0.9959024677
94,0.9906614594,0.9883244974,0.996024986
95,0.9894530518,0.9916174575,0.9962846902
96,0.9920828312,0.9899509876,0.9964171112
97,0.9905059403,0.9915210422,0.9964033731
98,0.992269794,0.9904762632,0.9960335672
99,0.9905076731,0.993076087,0.9958919539
100,0.9920942283,0.9863103732,0.9967811535
101,0.990191479,0.9907224697,0.9971989112
102,0.9914954573,0.9911115313,0.9961608979
103,0.992673381,0.9897732025,0.996296759
104,0.9900732337,0.9901660953,0.996053751
105,0.9915806437,0.9929730099,0.9959210415
106,0.9915051833,0.9923284015,0.9961672636
107,0.9914732462,0.9919989789,0.9960322494
108,0.9921255822,0.9921548149,0.9964307448
109,0.9917926657,0.9909043656,0.9968150032
110,0.9923317,0.9928162578,0.9965574376
111,0.9914454939,0.9912292746,0.996567095
112,0.9908025696,0.9923948124,0.9961803107
113,0.9906852569,0.9926995745,0.9968192107
114,0.9919210142,0.9936211267,0.996696872
115,0.9899248721,0.9930501534,0.9965866961
116,0.9910989633,0.9913999664,0.9968148979
117,0.9902805988,0.9922136816,0.9962086292
118,0.9911178651,0.9913965458,0.9960779854
119,0.9913169127,0.9924005903,0.9959546376
120,0.9917129602,0.9925924346,0.9968112069
121,0.9922500022,0.987713105,0.9962037724
122,0.9921335017,0.9909833462,0.9958227168
123,0.9919175751,0.9902082599,0.9968340579
124,0.9910878549,0.9919877209,0.9960844149
125,0.9914522541,0.992915429,0.9965906119
126,0.9916020558,0.991185028,0.9965859119
127,0.9921092128,0.9919084679,0.9963331013
128,0.9914074649,0.9922029356,0.9967121597
129,0.991572202,0.9927483418,0.9964684883
130,0.9927556005,0.9923876445,0.9967063216
131,0.9910522573,0.9935421817,0.9960937641
132,0.9929693092,0.9930196288,0.996581873
133,0.9928601342,0.9915037819,0.9964615376
134,0.9929547375,0.9922768148,0.9963486808
135,0.9913744477,0.993136074,0.9965986389
136,0.9929904166,0.9927129396,0.9963472483
137,0.9929006416,0.9930078063,0.995830936
138,0.9931709078,0.9923690843,0.9969781927
139,0.9921821072,0.9915940651,0.9960968281
140,0.9916837331,0.9926478842,0.9962262085
141,0.9906613568,0.9936404342,0.9960958073
142,0.9926727245,0.99214392,0.9960936363
143,0.9920274752,0.9919106843,0.9962248525
144,0.9924028893,0.9919478054,0.9962244825
145,0.992270499,0.9919315573,0.9964878057
146,0.993412292,0.9922078365,0.9967379646
147,0.9924153152,0.9937908836,0.9964796676
148,0.991705519,0.9915121096,0.9962485027
149,0.9918413332,0.9913666117,0.9963677929
150,0.9928961778,0.9932678243,0.9964815049
151,0.9927486884,0.9934223769,0.9967572902
152,0.9933340949,0.9935203322,0.9963974252
153,0.992778248,0.9933215555,0.9965231259
154,0.9926600904,0.9930175616,0.9965306182
155,0.9930123534,0.9932130748,0.9960341517
156,0.9929259568,0.9927960583,0.9962862339
157,0.9928118279,0.9929062261,0.996904572
158,0.9925730088,0.9926912243,0.9964156867
159,0.9929192461,0.9931599044,0.9960505414
160,0.9929339092,0.9932667617,0.9956920876
161,0.9928313606,0.9930588143,0.9960542073
162,0.9922804932,0.9926078927,0.995938941
163,0.9923873187,0.9929773561,0.9960616445
164,0.9926183282,0.9929529042,0.9961875374
165,0.9928568892,0.9927398684,0.9963105374
166,0.9924061319,0.9928495487,0.9958265242
167,0.9924208487,0.9929626639,0.9965548844
168,0.9924326255,0.9927475573,0.9960738111
169,0.9920899747,0.9930985691,0.9963194669
170,0.9920992444,0.9925349084,0.9961990644
171,0.9921010958,0.9923120129,0.9958372676
172,0.9917764354,0.9924410782,0.9957174002
173,0.9926594416,0.9923351844,0.9959630555
174,0.992105027,0.9924410782,0.9962032937
175,0.9920034443,0.9923358572,0.9960784321
176,0.9921301404,0.9922353838,0.9965819573
177,0.9921142615,0.991698742,0.996208236
178,0.9915864868,0.9923410115,0.9958425526
179,0.9921448116,0.9921237395,0.9958500606
180,0.9923588502,0.9920158513,0.9959746871
181,0.9919045088,0.9920332944,0.9961001419
182,0.9919200728,0.9920293473,0.9957350102
183,0.992157376,0.9922530364,0.9957331207
184,0.9919327625,0.9922602554,0.9959813037
185,0.992371311,0.9923857619,0.9959815578
186,0.9918261502,0.9924842228,0.9961107229
187,0.9916067721,0.9921578709,0.9955023511
188,0.9911723165,0.9918245274,0.9958608141
189,0.9917324065,0.9920543565,0.9959924516
190,0.9920725089,0.992061967,0.9958696895
191,0.9923941242,0.9920631188,0.9957488603
192,0.9916264746,0.9912848999,0.9957527436
193,0.9916322946,0.9917460952,0.9955142405
194,0.9914242323,0.9918423155,0.9961146454
195,0.991522653,0.9917422695,0.995873463
196,0.9913236074,0.9914091282,0.9959973724
197,0.9914333956,0.9914071371,0.9956383799
198,0.991419271,0.9918675597,0.9957624875
199,0.9915490791,0.9919868766,0.9960126878
200,0.99142076,0.9919831706,0.9960032865
201,0.9914289402,0.9916545772,0.9955354557
202,0.9913316167,0.9915537602,0.9960089326
203,0.9913303662,0.991653854,0.9960145628
204,0.9913143282,0.991333667,0.9958922277
205,0.9913338666,0.9916632468,0.9955348963
206,0.9912328387,0.9918879704,0.9961383779
207,0.990689826,0.9916706979,0.9958915835
208,0.9912373823,0.9915566834,0.9955415999
209,0.9914533876,0.9915707836,0.9956622529
210,0.9912489723,0.9915802384,0.9962648039
211,0.9909293192,0.9913506317,0.9957818418
212,0.991026319,0.9914625405,0.996137773
213,0.9914639628,0.9915749075,0.99590929
214,0.9912431811,0.9914657339,0.9956699723
215,0.9908389169,0.9915884637,0.9957923721
216,0.991367724,0.9916929714,0.9960358134
217,0.9908210343,0.9912540562,0.9960324731
218,0.99136822,0.9912693624,0.9957961764
219,0.9912507333,0.991149161,0.9959168136
220,0.9909259321,0.9914841111,0.9956794149
221,0.9909314023,0.9912733682,0.9959238023
222,0.9911432554,0.9913794187,0.9961614637
223,0.9909425828,0.9913848567,0.9958016738
224,0.9909451789,0.9911681857,0.9962830554
225,0.9912688054,0.9911560193,0.9958106742
226,0.9908376044,0.9911793089,0.9958029806
227,0.9913852947,0.9911803187,0.9961677879
228,0.9909464764,0.9911686919,0.9959243097
229,0.9911630634,0.9912766203,0.9959260844
230,0.9912897955,0.9908439612,0.9961656424
231,0.990848356,0.9908578373,0.9956881461
232,0.9911782401,0.9914008835,0.9959313992
233,0.9911812692,0.9911846078,0.9960561046
234,0.9911845483,0.9910822858,0.9959343038
235,0.9907470602,0.9909685386,0.9962920568
236,0.9909651195,0.9911793089,0.9962955073
237,0.9905264013,0.9909620781,0.9959367001
238,0.9909878015,0.990866195,0.9957048382
239,0.9908650886,0.9909695714,0.9960573277
240,0.9909823991,0.990862018,0.9961817934
241,0.9908582984,0.9908823445,0.9958279143
242,0.9905455954,0.9903433491,0.9958257186
243,0.9907610612,0.9911999638,0.9958200249
244,0.9903386021,0.991086362,0.9958262355
245,0.9905596038,0.9908760999,0.9961816752
246,0.9906731357,0.9907732437,0.9961814386
247,0.9905571823,0.9912074963,0.9960670853
248,0.9907758087,0.9911946833,0.9955972343
249,0.990563637,0.9906588337,0.995840527
250,0.9908812401,0.9907669248,0.9963067342
251,0.9900332534,0.990768242,0.9960708534
252,0.9911119432,0.9910101797,0.995949266
253,0.9903611266,0.9908893596,0.9959541456
254,0.990573839,0.9908875419,0.9958443729
255,0.990808819,0.9909891502,0.9959586395
256,0.9904669047,0.9908836444,0.9958395003
257,0.9906914297,0.990890917,0.9958391151
258,0.9910108815,0.9907785028,0.995844757
259,0.9907894607,0.9907811301,0.9957285174
260,0.9904761148,0.9907798167,0.9960789726
261,0.990490976,0.9910114588,0.9960823558
262,0.9907006818,0.9908997324,0.9958389867
263,0.990379726,0.9907908382,0.9960860947
264,0.9906021808,0.9908968822,0.9959654859
265,0.9904955601,0.9905867641,0.9962057664
266,0.9907038497,0.9906959951,0.9956105212
267,0.9901727136,0.9905848914,0.9959742897
268,0.9906091066,0.9906888513,0.9960917498
269,0.9902896525,0.9906941441,0.9958511498
270,0.9904998704,0.9905902401,0.9956243997
271,0.9902921269,0.9908151495,0.9957348228
272,0.9903887264,0.9905859616,0.9959745372
273,0.9906133635,0.9904672454,0.9960947511
274,0.9906192105,0.9905843562,0.9958587951
275,0.9901802284,0.9904859189,0.9958441167
276,0.9904017878,0.9902720938,0.9958590495
277,0.9900823138,0.9904891591,0.995976392
278,0.9903933563,0.9907120945,0.9957481602
279,0.9899764056,0.9906046512,0.9956336481
280,0.9901807846,0.9902864264,0.9958647643
281,0.9901924501,0.9908120198,0.9961044439
282,0.9899894286,0.9907181504,0.9962183366
283,0.9898765728,0.9906126384,0.9958685654
284,0.990211002,0.9905123154,0.9959860096
285,0.9899888631,0.9904072951,0.9961008596
286,0.9903113293,0.9902853254,0.9959592629
287,0.9901030324,0.9903988723,0.9958697044
288,0.9903091386,0.9896497936,0.9958727386
289,0.9903230875,0.9905155376,0.9955183639
290,0.9899846197,0.9904089236,0.995988714
291,0.9898868599,0.9906232668,0.9955253501
292,0.99020962,0.9899798855,0.9956428574
293,0.9898885724,0.9899708112,0.995881563
294,0.9902087906,0.9902011208,0.995873749
295,0.9903192624,0.9899852656,0.9958731176
296,0.9902151458,0.990317427,0.9956403253
297,0.9901086172,0.9904175996,0.9957580438
298,0.9902206655,0.9899835672,0.9956460515
299,0.9900125598,0.9901019947,0.9957544078
300,0.9899161773,0.9895676514,0.9958829462


==> supp_cifar0.4_csv/clean.tex <==
0,epochs,FINE,PASS,SmallLoss
0,50,0.83454,0.53659,0.63712
1,51,0.65982,0.538131,0.63012
2,52,0.65774,0.5360379999999999,0.64234
3,53,0.66592,0.538959,0.6265
4,54,0.66948,0.539396,0.63278
5,55,0.66684,0.5381079999999999,0.63008
6,56,0.6707,0.5396259999999999,0.6295
7,57,0.67228,0.5382229999999999,0.63032
8,58,0.6673,0.537326,0.62876
9,59,0.6616,0.541558,0.6295
10,60,0.67516,0.5396949999999999,0.62174
11,61,0.67078,0.53843,0.6248
12,62,0.6619,0.543697,0.6224
13,63,0.6694,0.5418799999999999,0.62122
14,64,0.6644,0.5388439999999999,0.6311
15,65,0.67022,0.541696,0.62692
16,66,0.64988,0.540408,0.6271
17,67,0.6621,0.541512,0.61612
18,68,0.65694,0.541604,0.62776
19,69,0.65914,0.5424779999999999,0.6177
20,70,0.65422,0.5418109999999999,0.62486
21,71,0.6584,0.54441,0.6236
22,72,0.64532,0.542018,0.61776
23,73,0.65758,0.543306,0.61572
24,74,0.6457,0.5444559999999999,0.61664
25,75,0.64806,0.5444559999999999,0.61732
26,76,0.6467,0.545445,0.619
27,77,0.64634,0.545445,0.62438
28,78,0.64194,0.545974,0.61562
29,79,0.64576,0.545974,0.62076
30,80,0.63418,0.5456289999999999,0.61418
31,81,0.6408,0.5477909999999999,0.61982
32,82,0.63274,0.547055,0.61392
33,83,0.6369,0.547538,0.61644
34,84,0.64078,0.548389,0.62216
35,85,0.63444,0.5471929999999999,0.61552
36,86,0.63812,0.548044,0.6199
37,87,0.63276,0.5476989999999999,0.61658
38,88,0.6347,0.5490559999999999,0.62132
39,89,0.62824,0.549079,0.61854
40,90,0.63796,0.548665,0.6164
41,91,0.63618,0.5487799999999999,0.62084
42,92,0.63066,0.548573,0.61788
43,93,0.6304,0.551195,0.61298
44,94,0.62986,0.547492,0.61984
45,95,0.63166,0.548642,0.61742
46,96,0.6257,0.55062,0.61666
47,97,0.62792,0.5499299999999999,0.61588
48,98,0.62174,0.5514709999999999,0.6119
49,99,0.62972,0.55085,0.61648
50,100,0.62126,0.550505,0.61616
51,101,0.62582,0.5510569999999999,0.61544
52,102,0.6237,0.552368,0.61178
53,103,0.62474,0.5521379999999999,0.61518
54,104,0.62304,0.552828,0.60994
55,105,0.62656,0.552345,0.61634
56,106,0.6203,0.5508959999999999,0.61724
57,107,0.62562,0.5516779999999999,0.60988
58,108,0.62456,0.5542079999999999,0.61082
59,109,0.62408,0.5535869999999999,0.61192
60,110,0.61882,0.551931,0.61418
61,111,0.62456,0.554484,0.61074
62,112,0.62412,0.55223,0.6192
63,113,0.6216,0.550666,0.6108
64,114,0.62046,0.5498609999999999,0.61854
65,115,0.62118,0.553771,0.60592
66,116,0.61474,0.552667,0.61134
67,117,0.61948,0.5558409999999999,0.61032
68,118,0.62108,0.552299,0.60456
69,119,0.62464,0.555634,0.61422
70,120,0.61838,0.553403,0.61608
71,121,0.62152,0.5557949999999999,0.61816
72,122,0.60438,0.556508,0.60884
73,123,0.61768,0.556784,0.6092
74,124,0.6098,0.556485,0.61168
75,125,0.6154,0.555864,0.60322
76,126,0.60458,0.5548289999999999,0.61292
77,127,0.61008,0.556117,0.61202
78,128,0.6163,0.5568069999999999,0.61416
79,129,0.60786,0.555565,0.60528
80,130,0.61624,0.556002,0.61104
81,131,0.60986,0.556715,0.61022
82,132,0.60792,0.557014,0.61322
83,133,0.61192,0.5569679999999999,0.60532
84,134,0.61518,0.559176,0.60728
85,135,0.61248,0.557589,0.59948
86,136,0.61042,0.560832,0.6083
87,137,0.61502,0.5584629999999999,0.59622
88,138,0.61196,0.5585319999999999,0.60444
89,139,0.60882,0.5584629999999999,0.59684
90,140,0.6097,0.558394,0.59592
91,141,0.61038,0.560326,0.60008
92,142,0.60512,0.559889,0.60716
93,143,0.6109,0.560487,0.60516
94,144,0.6108,0.5597279999999999,0.60508
95,145,0.60074,0.560211,0.59228
96,146,0.613,0.561407,0.601
97,147,0.60264,0.559705,0.5939
98,148,0.6069,0.5606939999999999,0.60126
99,149,0.60994,0.5595209999999999,0.5902
100,150,0.60812,0.561522,0.60266
101,151,0.61156,0.5628099999999999,0.60662
102,152,0.61284,0.563615,0.6079
103,153,0.61466,0.563684,0.61174
104,154,0.61736,0.56511,0.60986
105,155,0.61836,0.5655469999999999,0.61134
106,156,0.61414,0.5660069999999999,0.61348
107,157,0.61592,0.565731,0.6119
108,158,0.61526,0.5664669999999999,0.61358
109,159,0.61708,0.56718,0.61284
110,160,0.6158,0.566651,0.61232
111,161,0.61704,0.567686,0.61088
112,162,0.61874,0.5682839999999999,0.61308
113,163,0.6162,0.5687209999999999,0.61376
114,164,0.61776,0.568974,0.6148
115,165,0.61812,0.5692499999999999,0.61402
116,166,0.62046,0.5687899999999999,0.614
117,167,0.61794,0.568583,0.61474
118,168,0.6185,0.569457,0.61414
119,169,0.61692,0.571665,0.61252
120,170,0.61668,0.570032,0.61288
121,171,0.61708,0.569641,0.61296
122,172,0.61616,0.570561,0.6129
123,173,0.61708,0.5708599999999999,0.61228
124,174,0.6169,0.570676,0.61472
125,175,0.61808,0.57017,0.61468
126,176,0.61818,0.571688,0.61382
127,177,0.6195,0.571642,0.61408
128,178,0.61732,0.5720559999999999,0.61366
129,179,0.61902,0.5724469999999999,0.61464
130,180,0.61854,0.572079,0.61562
131,181,0.618,0.572746,0.61416
132,182,0.62016,0.572861,0.61292
133,183,0.61802,0.573206,0.61492
134,184,0.61926,0.572171,0.61304
135,185,0.61844,0.5729759999999999,0.61504
136,186,0.61744,0.5734819999999999,0.61348
137,187,0.61858,0.573827,0.61546
138,188,0.61822,0.573712,0.61518
139,189,0.61844,0.5734589999999999,0.61442
140,190,0.618,0.5734589999999999,0.61476
141,191,0.61926,0.5735279999999999,0.61572
142,192,0.61918,0.5751379999999999,0.61498
143,193,0.61914,0.5747239999999999,0.61386
144,194,0.61872,0.5753449999999999,0.61376
145,195,0.61938,0.5753449999999999,0.61374
146,196,0.62026,0.5753219999999999,0.6158
147,197,0.61938,0.5751149999999999,0.61414
148,198,0.6209,0.574885,0.61558
149,199,0.62002,0.57569,0.61508
150,200,0.6208,0.5759659999999999,0.61616
151,201,0.62036,0.577231,0.61588
152,202,0.61946,0.576449,0.6142
153,203,0.6193,0.5763799999999999,0.61452
154,204,0.61932,0.575897,0.61484
155,205,0.61984,0.5767479999999999,0.61362
156,206,0.62048,0.577668,0.61612
157,207,0.61998,0.5775069999999999,0.61438
158,208,0.62016,0.577231,0.61614
159,209,0.62038,0.5772539999999999,0.61564
160,210,0.62118,0.5781509999999999,0.61554
161,211,0.62014,0.5783349999999999,0.61556
162,212,0.6198,0.577438,0.61624
163,213,0.62074,0.577231,0.61618
164,214,0.6213,0.577852,0.61432
165,215,0.6213,0.578243,0.6151
166,216,0.62078,0.578243,0.61574
167,217,0.62064,0.578887,0.61584
168,218,0.62164,0.578887,0.6157
169,219,0.62078,0.579255,0.61744
170,220,0.62142,0.5793699999999999,0.61676
171,221,0.62108,0.579186,0.6167
172,222,0.6204,0.5794159999999999,0.61626
173,223,0.62078,0.5796,0.61604
174,224,0.62124,0.5794159999999999,0.61658
175,225,0.62186,0.580152,0.61718
176,226,0.62262,0.579508,0.61686
177,227,0.62142,0.5811179999999999,0.61772
178,228,0.62022,0.580773,0.61622
179,229,0.62126,0.5808189999999999,0.617
180,230,0.62146,0.580543,0.61724
181,231,0.62208,0.580152,0.61696
182,232,0.62284,0.581371,0.6153
183,233,0.62186,0.5811179999999999,0.61722
184,234,0.62196,0.581463,0.6173
185,235,0.622,0.580359,0.61696
186,236,0.622,0.581141,0.61806
187,237,0.6212,0.581187,0.61764
188,238,0.62292,0.581693,0.6177
189,239,0.6218,0.5813479999999999,0.61868
190,240,0.62178,0.5818309999999999,0.61788
191,241,0.62326,0.5819689999999998,0.61764
192,242,0.62214,0.5815779999999999,0.618
193,243,0.6228,0.582291,0.61782
194,244,0.62246,0.5822679999999999,0.61706
195,245,0.6239,0.5820609999999999,0.6185
196,246,0.62178,0.5826359999999999,0.61806
197,247,0.62282,0.582452,0.61792
198,248,0.62226,0.581992,0.61782
199,249,0.62328,0.582291,0.61692
200,250,0.62484,0.5831189999999999,0.61738
201,251,0.62404,0.582843,0.61826
202,252,0.62436,0.58305,0.61848
203,253,0.6237,0.5828889999999999,0.61776
204,254,0.62366,0.583648,0.61914
205,255,0.62294,0.583579,0.61776
206,256,0.62326,0.584062,0.61812
207,257,0.62316,0.583464,0.61926
208,258,0.62408,0.584453,0.61864
209,259,0.62498,0.583832,0.61832
210,260,0.62474,0.584361,0.61966
211,261,0.62244,0.5842689999999999,0.62066
212,262,0.62464,0.5854189999999999,0.61932
213,263,0.624,0.584683,0.61972
214,264,0.62364,0.5848439999999999,0.6204
215,265,0.62256,0.5844299999999999,0.61978
216,266,0.62252,0.584867,0.62002
217,267,0.624,0.5842229999999999,0.61926
218,268,0.6242,0.58466,0.6203
219,269,0.62432,0.58489,0.61982
220,270,0.62358,0.585235,0.62038
221,271,0.62388,0.585741,0.62036
222,272,0.62428,0.5864309999999999,0.61942
223,273,0.62378,0.5858559999999999,0.61926
224,274,0.6242,0.585718,0.62114
225,275,0.62578,0.5861779999999999,0.62068
226,276,0.62454,0.585994,0.6206
227,277,0.62578,0.5861779999999999,0.61942
228,278,0.62462,0.5854649999999999,0.61886
229,279,0.62484,0.5864539999999999,0.62092
230,280,0.62542,0.5857870000000001,0.62098
231,281,0.62606,0.586661,0.62032
232,282,0.62568,0.586868,0.62098
233,283,0.62652,0.586776,0.62138
234,284,0.62504,0.5861779999999999,0.62044
235,285,0.6255,0.5864769999999999,0.62134
236,286,0.6256,0.587305,0.621
237,287,0.62484,0.5868909999999999,0.6212
238,288,0.6246,0.587397,0.62276
239,289,0.62536,0.587673,0.62122
240,290,0.62632,0.5877189999999999,0.62172
241,291,0.6264,0.587696,0.62108
242,292,0.62552,0.588064,0.62154
243,293,0.6263,0.588156,0.6216
244,294,0.6256,0.58788,0.62172
245,295,0.62656,0.58834,0.62364
246,296,0.6271,0.5883629999999999,0.62198
247,297,0.62616,0.5886389999999999,0.62224
248,298,0.62666,0.589214,0.62122
249,299,0.62494,0.588271,0.62258
250,300,0.6263,0.588846,0.6225

==> supp_cifar0.4_csv/f1.tex <==
epochs,FINE,PASS,SmallLoss
50,0.6652859047,0.8681156189,0.8220862827
51,0.7350587827,0.8696238493,0.8205202436
52,0.781206983,0.8678811882,0.8263787371
53,0.7902059068,0.870383718,0.8248921435
54,0.8043044945,0.870100836,0.8235606705
55,0.8031297992,0.8696483382,0.8237605565
56,0.8077703925,0.8708583934,0.8239450008
57,0.8110127927,0.8697995457,0.8239805872
58,0.8059240959,0.8688384753,0.8240582955
59,0.8120927197,0.8725801947,0.8263223887
60,0.8064915565,0.8706482453,0.8281770849
61,0.811301944,0.8697159659,0.826776563
62,0.8086891182,0.8746213785,0.8248685441
63,0.8109763955,0.87310173,0.8274309619
64,0.8105670851,0.8701870643,0.8255617039
65,0.8118504646,0.872797236,0.8303532913
66,0.8116277891,0.8714377764,0.825935419
67,0.8130501513,0.8725836899,0.8301272902
68,0.8174811165,0.8728952712,0.8263899301
69,0.8154664247,0.8732379276,0.8289102589
70,0.813201601,0.8736759231,0.8268317552
71,0.8119902122,0.8758151641,0.8277224899
72,0.8157571845,0.8736372143,0.8284687775
73,0.8135178566,0.8747200616,0.8281095404
74,0.8118866388,0.875811526,0.828196694
75,0.8165777257,0.8755389087,0.8273733749
76,0.818008095,0.876891177,0.8277058981
77,0.8136139801,0.876891177,0.82741481
78,0.8122344835,0.8765084186,0.8284764284
79,0.8144547974,0.8769622938,0.8279968783
80,0.8000821512,0.8763770262,0.8245723598
81,0.8127887855,0.878561885,0.8314027935
82,0.8167458405,0.8776693517,0.8267829934
83,0.8149152005,0.8782424333,0.8305383871
84,0.8149624502,0.8791475418,0.8325258909
85,0.8171823297,0.8780210306,0.8286901866
86,0.8183069501,0.8787452187,0.8315147151
87,0.8227695372,0.8786600874,0.8259227863
88,0.8193676252,0.8800214357,0.8274851533
89,0.819899971,0.8797703372,0.8281968542
90,0.8184594281,0.879668656,0.8238066503
91,0.8160474399,0.8794552316,0.8326475236
92,0.8160332149,0.8795856167,0.8264402859
93,0.8119285262,0.8814949598,0.826829272
94,0.816987174,0.8783368717,0.8290924901
95,0.8184550877,0.8792400336,0.833014662
96,0.8182738348,0.8815661394,0.835534625
97,0.817946664,0.8806733454,0.8341239115
98,0.8172165642,0.8819240132,0.8303208921
99,0.8118628809,0.8813204273,0.8309201875
100,0.8199193096,0.8807836838,0.8361486258
101,0.8203115391,0.8813256184,0.8380602074
102,0.8191089605,0.8826390845,0.8379563014
103,0.8209030594,0.882703965,0.8346294002
104,0.8217569293,0.8831421326,0.8319271145
105,0.8225434793,0.8823923963,0.8353546586
106,0.8225253358,0.8812713014,0.8364528706
107,0.8230393757,0.8821552321,0.8395608675
108,0.8242973246,0.8845136671,0.8372607194
109,0.8213914867,0.883912656,0.8352695525
110,0.8243525383,0.8826538277,0.8379373917
111,0.8264589458,0.8847153693,0.8393896429
112,0.8234746537,0.8830126449,0.8341576008
113,0.8229305153,0.8812454042,0.8383240926
114,0.8250327386,0.8804753359,0.8349663917
115,0.8243667341,0.884393657,0.8366978563
116,0.8302852153,0.883178573,0.8296076826
117,0.8214226664,0.8860628948,0.8416711834
118,0.8252253317,0.8830293325,0.8358961791
119,0.8203565823,0.8858781753,0.8363958366
120,0.8268061452,0.8838382268,0.8353835547
121,0.8215649934,0.8858864907,0.8376447457
122,0.8322523512,0.8862968994,0.836390758
123,0.8273038545,0.8869487146,0.8377309737
124,0.8314676614,0.8867724968,0.8368216287
125,0.828328314,0.8860382963,0.8396655299
126,0.8328273433,0.885068944,0.8404377156
127,0.8278743349,0.8861737585,0.8398386053
128,0.8354123011,0.8870142982,0.8364558751
129,0.834453075,0.8856360839,0.8408817535
130,0.8283411374,0.8859358441,0.8384302992
131,0.8333758233,0.8867068629,0.8396820922
132,0.8330775317,0.8869281391,0.8384769873
133,0.8298187158,0.8868871675,0.8419305651
134,0.8290440404,0.8891205675,0.8444475199
135,0.8333791274,0.8873498945,0.8473644341
136,0.8305024615,0.8904532366,0.8430989471
137,0.8288573227,0.8883072913,0.8482175012
138,0.8317415833,0.8887740251,0.8395168922
139,0.8332969237,0.8882172016,0.8472218545
140,0.8348105563,0.8886964971,0.851524088
141,0.8326243373,0.8900501635,0.8483540325
142,0.8374079598,0.8894828911,0.840955835
143,0.8357310684,0.8902827499,0.8505553219
144,0.8319736282,0.8892501187,0.843342996
145,0.8383442669,0.8899482824,0.8454369029
146,0.8348235599,0.8910518983,0.8466224503
147,0.8364165943,0.8894997835,0.8475472907
148,0.8353019763,0.8904210432,0.8435772719
149,0.8341451394,0.8893816216,0.8517986399
150,0.8370951909,0.8909287747,0.8479681324
151,0.8377322505,0.8922013119,0.851589804
152,0.8364861719,0.8927764532,0.8500011588
153,0.8365122445,0.8930617699,0.8495290747
154,0.8371183728,0.8940475989,0.8500152363
155,0.83658097,0.8945213957,0.847106067
156,0.8374948094,0.8948805618,0.8481035567
157,0.8357914101,0.8946830321,0.8490941792
158,0.8365275799,0.895194637,0.8476922246
159,0.8369373635,0.8957750577,0.84891041
160,0.8371409468,0.8952664212,0.8495572378
161,0.8369773084,0.8961735617,0.8476912444
162,0.8375436942,0.8969208689,0.8484334238
163,0.8370100302,0.8971687314,0.8494054083
164,0.8385610636,0.897524135,0.8499320571
165,0.8374338999,0.8977205095,0.8499919996
166,0.8378587239,0.897094782,0.8506319094
167,0.8382659368,0.8972718987,0.8495290196
168,0.8385503114,0.8979460288,0.8505277314
169,0.8381725064,0.8998259003,0.850981572
170,0.8373369841,0.8983136876,0.8504584461
171,0.8384733675,0.8978382586,0.8505317606
172,0.8371268638,0.8988644348,0.8501666835
173,0.838281313,0.8989461931,0.8503348919
174,0.8373091406,0.8988752519,0.850323105
175,0.8380876486,0.898434071,0.8516024263
176,0.8380261035,0.899577847,0.8505445776
177,0.8373988408,0.8993144414,0.8502792242
178,0.8390781998,0.8999873431,0.8523355303
179,0.8378009429,0.900416606,0.8510239089
180,0.8378199931,0.9000073459,0.8504886174
181,0.8375153443,0.900497817,0.8508945149
182,0.8386556345,0.9005084364,0.852046148
183,0.8364215018,0.9009865936,0.8513960294
184,0.8368719393,0.8999980242,0.8526602648
185,0.8386102821,0.9010101075,0.8515057083
186,0.8377293602,0.9013154011,0.8526361458
187,0.8377417155,0.9015254344,0.8528955436
188,0.8386767524,0.9012918277,0.8520980318
189,0.8391474283,0.9009830528,0.85256532
190,0.8375537069,0.9009830528,0.8531083358
191,0.840091686,0.9009983134,0.8542553289
192,0.8393279812,0.9027504211,0.8532704714
193,0.8399432824,0.9021244581,0.852130859
194,0.8392126644,0.9024837878,0.853977993
195,0.839511449,0.9027066512,0.8529126702
196,0.8398965125,0.9026421745,0.8531283788
197,0.8395881348,0.9025521822,0.8538985122
198,0.8391806966,0.9022638913,0.85397281
199,0.8393317267,0.9029605265,0.8529357912
200,0.8405825569,0.9031991694,0.8526057148
201,0.8391453833,0.9042470997,0.8547883364
202,0.8395464797,0.9035720012,0.8524029894
203,0.8395914503,0.9036460323,0.8531990775
204,0.8408371858,0.9030504022,0.8543824245
205,0.8383621191,0.9040529103,0.8555963091
206,0.8389872938,0.9044904724,0.8533815322
207,0.8397548958,0.9042626098,0.8538463058
208,0.8398815247,0.9040245007,0.8540575438
209,0.8398148873,0.9041779022,0.8539113758
210,0.8389396236,0.9051292652,0.855253137
211,0.8399398389,0.9051097838,0.8544966911
212,0.8389767354,0.9042921181,0.8541486734
213,0.8402595008,0.904291622,0.8533201807
214,0.8392408447,0.9046936071,0.8550710457
215,0.8393939128,0.9049415525,0.8543096299
216,0.8402961205,0.9050305364,0.8540799852
217,0.8404360943,0.905629503,0.8546744488
218,0.8405852655,0.9055405523,0.8560187707
219,0.83945362,0.9058126979,0.8545451842
220,0.8390828833,0.905911604,0.85237972
221,0.8409919811,0.9059756839,0.8536394253
222,0.8410594143,0.9059511615,0.8537412882
223,0.8407174821,0.9064205634,0.8553987399
224,0.8411383274,0.9060400819,0.8551548854
225,0.8405185535,0.9067170137,0.8535354349
226,0.8406394043,0.9060747251,0.8552162614
227,0.8404988775,0.9074571921,0.8546839552
228,0.8409712948,0.9070279766,0.8556787933
229,0.8396251894,0.9072451352,0.8552662795
230,0.8408800167,0.9071415806,0.8557553747
231,0.8411788454,0.9065392526,0.8529871636
232,0.8409168326,0.9075853063,0.8555381598
233,0.840633352,0.9073239533,0.8557371873
234,0.8401126158,0.9077529806,0.8545724264
235,0.8413353664,0.9068058933,0.8536829559
236,0.8406848127,0.9076545771,0.8545294915
237,0.839991321,0.9074275396,0.8541474317
238,0.8413340105,0.9080388829,0.8545111748
239,0.8410377573,0.9078320406,0.8547454818
240,0.8412874238,0.9080683118,0.854945404
241,0.8400391669,0.9083196913,0.8559256384
242,0.8413867389,0.9077627393,0.8544749272
243,0.8414539077,0.9084622199,0.8547749054
244,0.8402255264,0.9083093855,0.8563655458
245,0.8418840689,0.9082653014,0.8547749874
246,0.8419382817,0.9086687197,0.8554182045
247,0.8411279906,0.9084668897,0.8545567148
248,0.8407694182,0.908206212,0.8561278831
249,0.841394974,0.908329076,0.8562769548
250,0.8412515374,0.9089931044,0.8563855654
251,0.8409039342,0.9088458009,0.8544023322
252,0.8405849169,0.9089341055,0.8541775768
253,0.8419309978,0.9090182425,0.8537157249
254,0.8412448721,0.9094895605,0.8541598856
255,0.8423466668,0.9093862674,0.8558413622
256,0.841338496,0.9098431155,0.8564777234
257,0.8420119133,0.9094654003,0.8545004179
258,0.8409022318,0.9099995374,0.8550952986
259,0.8422569961,0.9094250418,0.8553453441
260,0.8423438991,0.9100539944,0.8547478973
261,0.8411634009,0.9099754808,0.8543060367
262,0.8427111334,0.9109560896,0.856330487
263,0.8411347959,0.9105059691,0.8558826771
264,0.8419145033,0.9104660058,0.8549566244
265,0.8420764134,0.9102015172,0.8542011791
266,0.8404333157,0.9104856176,0.8554988874
267,0.842701305,0.9098918929,0.8536902373
268,0.8421193184,0.9103977183,0.8559070732
269,0.8441012253,0.9104609199,0.854623141
270,0.8421273554,0.9106221173,0.8556325053
271,0.8429742152,0.9112746307,0.8549203425
272,0.8424596444,0.9115962378,0.8536042189
273,0.841430755,0.9112839756,0.8555038777
274,0.8420429131,0.9111664723,0.8546642797
275,0.8413828644,0.9116023254,0.8542085929
276,0.8413216694,0.9113128975,0.8558319286
277,0.8418023602,0.9115137778,0.8559965074
278,0.8426547252,0.9109509838,0.8576904273
279,0.8424349623,0.9117928633,0.8560447766
280,0.8420469119,0.9113580838,0.8553283091
281,0.8412564743,0.911791869,0.855693799
282,0.8420164951,0.9121448917,0.855675147
283,0.8415987866,0.9119781689,0.8552669628
284,0.8417009038,0.9114695051,0.8551085561
285,0.8429592824,0.911768161,0.8553462848
286,0.8425159781,0.9122950223,0.8565798485
287,0.8421676861,0.9119874298,0.8549883011
288,0.8432859428,0.9125058937,0.8553999695
289,0.8427937448,0.9126518112,0.8558540277
290,0.8424842494,0.9126466383,0.8564608174
291,0.8420994865,0.9128040328,0.8555730644
292,0.8419471682,0.9128952593,0.8558741219
293,0.8429236752,0.9132828571,0.8555432675
294,0.8425541358,0.9128717664,0.8564608174
295,0.842893051,0.9131736364,0.8555035417
296,0.8418594416,0.9133699963,0.855425264
297,0.8424150253,0.913338788,0.8556990947
298,0.8428314231,0.9139586614,0.8551990369
299,0.8407321222,0.9132477509,0.855929721
300,0.8425041957,0.9136910628,0.8552031857

==> supp_cifar0.4_csv/precision.tex <==
epochs,FINE,PASS,SmallLoss
50,0.5347406448,0.9916904396,0.7686705335
51,0.6645763341,0.9918422786,0.7715507375
52,0.7131291412,0.9920677621,0.7699259183
53,0.717910072,0.9918547769,0.7787139587
54,0.7305012377,0.9909030428,0.773087549
55,0.7307644092,0.9919059927,0.7750882735
56,0.7334026109,0.9916731859,0.7756740583
57,0.7358699361,0.9919717684,0.7751674339
58,0.7334012325,0.9917659388,0.7762905024
59,0.7430854624,0.9916391637,0.7782546361
60,0.7296101242,0.9912911079,0.7855510331
61,0.7370108589,0.991590729,0.7819207414
62,0.739358514,0.9917987593,0.7814742063
63,0.7374520042,0.9919621823,0.7850921812
64,0.7398757758,0.991725102,0.7763633167
65,0.7378944328,0.9917685482,0.784381275
66,0.7495513125,0.9914938707,0.779445335
67,0.7437947943,0.9917021059,0.7916244778
68,0.7514787726,0.9920217506,0.7794954171
69,0.7480576178,0.9913991797,0.789168975
70,0.7486005194,0.9928522178,0.7819401457
71,0.7448495574,0.9925694757,0.7837740285
72,0.7567228944,0.9925367661,0.7886406534
73,0.7469351364,0.9924274639,0.7896799459
74,0.7523753557,0.9925067586,0.7891275759
75,0.7559032177,0.9921267555,0.7877427537
76,0.7582612166,0.9927732434,0.7869344615
77,0.753815655,0.9927732434,0.7829042133
78,0.7550728403,0.9915803418,0.7901555612
79,0.7550661516,0.99221174,0.7860311502
80,0.7469448575,0.991827719,0.7868622877
81,0.7563765751,0.9921745623,0.7904271211
82,0.7657641845,0.9918489631,0.7894884463
83,0.7611174914,0.992045019,0.791851914
84,0.7587104859,0.9922459486,0.7900298396
85,0.7651330765,0.9921660329,0.7904622679
86,0.7639771928,0.9921152534,0.7904942663
87,0.7722537849,0.9924250837,0.7866636525
88,0.7673179539,0.9926321954,0.7850825232
89,0.7721315625,0.9922556673,0.7877953978
90,0.7642430422,0.9926269578,0.7844590738
91,0.7627931456,0.9921886281,0.7910828432
92,0.7663504443,0.9926257244,0.7863238536
93,0.7620875122,0.9920351085,0.7902074642
94,0.7679060155,0.9922332777,0.7878732643
95,0.7683130384,0.9920609836,0.7938915418
96,0.7720577489,0.9928410005,0.7972149144
97,0.7702250652,0.9924557362,0.7962112194
98,0.7735696846,0.9922891711,0.7948490503
99,0.7624588317,0.9922179051,0.7922450571
100,0.7768485728,0.9918999062,0.7982510483
101,0.7741937146,0.9919705573,0.8008842929
102,0.7743097281,0.9921768137,0.8034203583
103,0.7755637968,0.9925482905,0.7972707501
104,0.7776453999,0.9923080495,0.798050595
105,0.7761255018,0.9918644049,0.7972441756
106,0.7803578679,0.9920933798,0.7978165247
107,0.7772979042,0.9923545619,0.8066014977
108,0.7793864167,0.9925138246,0.8033469866
109,0.7765417623,0.9924431522,0.8003302265
110,0.7833837009,0.9927329718,0.8016567354
111,0.7817459966,0.992455346,0.8057779856
112,0.7787872721,0.9928618221,0.7938949148
113,0.7799100243,0.9923405475,0.8045463197
114,0.782995978,0.9922666525,0.7952523924
115,0.7817703644,0.9928816382,0.8063328287
116,0.7927872452,0.9925554053,0.7944605068
117,0.7797132014,0.9926598597,0.8086325737
118,0.7827797899,0.9928002556,0.8064483553
119,0.7750357943,0.9926571319,0.799917627
120,0.7863862321,0.9925652815,0.7974617753
121,0.7784708666,0.9924730971,0.7984782571
122,0.8025078362,0.9921729027,0.8038290461
123,0.7874229691,0.9927342084,0.8050599641
124,0.797650485,0.9928542834,0.8022306671
125,0.7901566153,0.9925981155,0.8116893883
126,0.8030034019,0.9925221825,0.8053498207
127,0.7934527731,0.9924774443,0.8053403568
128,0.7973458156,0.9927964555,0.8000274655
129,0.8023965769,0.9924079164,0.8115033963
130,0.7895776236,0.9922898281,0.8044888929
131,0.7997308441,0.9924855043,0.8064863916
132,0.8008170449,0.9924276159,0.8029514297
133,0.7942868252,0.9924269921,0.8126510761
134,0.7911028896,0.9928269003,0.8140025469
135,0.7978345587,0.9923117159,0.8232511112
136,0.7961275601,0.9926635216,0.8117279871
137,0.791010006,0.9925707202,0.8267734825
138,0.7963918038,0.9931274748,0.8106022678
139,0.8004023261,0.9924472135,0.8251525894
140,0.8014457898,0.9931875683,0.8307785667
141,0.798516107,0.9927184682,0.823906197
142,0.8077352625,0.9924664012,0.8101783584
143,0.8015949358,0.9928436381,0.8224767
144,0.7974878143,0.992341021,0.8144191462
145,0.8120929252,0.9927169771,0.8267262081
146,0.7990626227,0.9927938947,0.8212331789
147,0.8084830279,0.9927104091,0.8278467903
148,0.804053332,0.9927847534,0.8175912854
149,0.800529223,0.9927696639,0.8356895307
150,0.8051561045,0.9924882548,0.821475122
151,0.8033411421,0.9926892423,0.8225270441
152,0.8010246581,0.9925160796,0.8197689105
153,0.7997392895,0.9928229335,0.8163580886
154,0.798475937,0.9924748018,0.8183078597
155,0.7971707904,0.9926025641,0.8139474778
156,0.8012040287,0.9925476281,0.8134767103
157,0.7980367948,0.9926049641,0.8157529356
158,0.7993249576,0.9924319044,0.8129443826
159,0.7984755849,0.9923805937,0.8148500151
160,0.7996167586,0.9923126446,0.8159581106
161,0.7985483039,0.992326624,0.8149436839
162,0.7979637427,0.9926381038,0.8141401016
163,0.7991851068,0.9924618228,0.8147216688
164,0.7997853435,0.9926470096,0.8145414577
165,0.798283197,0.9925899782,0.8151837086
166,0.7970934833,0.9922808553,0.8159121622
167,0.7993306998,0.9927632899,0.8141366509
168,0.7992458839,0.9926532308,0.8156924427
169,0.7999560644,0.9926212041,0.817400813
170,0.7992033707,0.9924791157,0.8165487279
171,0.8001744202,0.9922923572,0.8165711936
172,0.7993430801,0.9926069621,0.8162080587
173,0.7999619519,0.9923691787,0.8168567666
174,0.7990152771,0.9924875815,0.8150361239
175,0.7990338973,0.9924809314,0.8164916351
176,0.7988946699,0.9922595682,0.8159479353
177,0.7972651331,0.9919573803,0.8154596641
178,0.8006717782,0.9923850916,0.8180654614
179,0.7980489201,0.9925107644,0.8158762326
180,0.7984108768,0.992385397,0.8145578874
181,0.7984585769,0.9922738295,0.8160867089
182,0.7981838319,0.9921549978,0.8182926332
183,0.7972361827,0.99240033,0.8160842789
184,0.7968539136,0.9922660853,0.8188895131
185,0.7993548521,0.992698241,0.8161179429
186,0.7990942972,0.9925242467,0.8185349913
187,0.7982960132,0.9924085334,0.8173567525
188,0.7995850439,0.9922267031,0.8166747191
189,0.7999482767,0.9921030337,0.8177579945
190,0.7985009587,0.9921030337,0.8181118361
191,0.8004071263,0.9920438676,0.8186801785
192,0.7996208148,0.9925457177,0.81812973
193,0.800328679,0.9921803609,0.8176884574
194,0.7998208353,0.9919490846,0.8198254925
195,0.7996811573,0.9922487084,0.8186504712
196,0.799481318,0.9921884674,0.8173651752
197,0.7997658079,0.9923055725,0.8194539121
198,0.7982393303,0.992182545,0.818468799
199,0.7990285422,0.9921934476,0.8176825103
200,0.7998551277,0.9921971787,0.816517667
201,0.798582228,0.9921545013,0.8191559654
202,0.7996629654,0.9921438864,0.817739956
203,0.7998263501,0.9923224161,0.8183909761
204,0.8011876899,0.9920765086,0.8194740043
205,0.7980867196,0.9924468835,0.8217385681
206,0.7983230578,0.9919813727,0.8174111152
207,0.7995236993,0.9918597568,0.8192172401
208,0.7995356965,0.9918558753,0.8181494025
209,0.7993062501,0.9920353602,0.8183559422
210,0.7977761314,0.992286231,0.8199260817
211,0.7996142051,0.9920502076,0.8190676751
212,0.7987929483,0.9919781874,0.8181771073
213,0.7995414637,0.9922142338,0.8172985457
214,0.7980232307,0.9920435805,0.820629399
215,0.7981918121,0.991929706,0.8191998916
216,0.7995535092,0.9920489461,0.8184699388
217,0.7998070058,0.9921173255,0.8190586074
218,0.7992639819,0.9919982126,0.8206614121
219,0.7986248768,0.9919437672,0.8177345276
220,0.7977646648,0.991945362,0.8158249372
221,0.8001081598,0.9922404454,0.8172709422
222,0.8006647257,0.9919459997,0.8177085685
223,0.8000180589,0.9923649598,0.8197180011
224,0.8001561804,0.9920649997,0.8190469998
225,0.7990352226,0.9921344679,0.8168022174
226,0.7986327398,0.9920067642,0.818908693
227,0.7993242338,0.9920288503,0.8176831114
228,0.8006953482,0.9918460534,0.8198969468
229,0.7984747842,0.992084116,0.8188611289
230,0.7997158772,0.9922585359,0.8192287227
231,0.7996070554,0.9918967683,0.8163538641
232,0.7987831705,0.9919137126,0.8204221317
233,0.7991616352,0.991850881,0.8192232213
234,0.7985177711,0.9920335671,0.8178678075
235,0.7998358991,0.9920184535,0.8171280803
236,0.7991195262,0.9922664812,0.8172617446
237,0.7989205075,0.9919111595,0.8171451245
238,0.7991858277,0.99215525,0.8175056236
239,0.7996493731,0.9922692277,0.8170474562
240,0.7999385112,0.9920385923,0.8178563687
241,0.79752306,0.9922182069,0.8191234733
242,0.7997936273,0.9919165829,0.8172450937
243,0.7994022258,0.9920448648,0.8177108116
244,0.798289949,0.9918669317,0.8200410692
245,0.7991019293,0.9920417298,0.8172120703
246,0.8006555613,0.9919312217,0.8182499788
247,0.7990295465,0.991869494,0.8173947384
248,0.7990293464,0.9920407888,0.8192159935
249,0.7989996827,0.9918672521,0.8200458192
250,0.7977488602,0.9918196527,0.8198271237
251,0.7979267291,0.9919340795,0.8169737535
252,0.7973524414,0.9918186873,0.816562862
253,0.7992939555,0.9921121529,0.8165770124
254,0.7985677708,0.9918861094,0.8160607479
255,0.8002860216,0.9918260831,0.8189413342
256,0.7989516299,0.9918918451,0.819384425
257,0.7997626903,0.9920608152,0.8163512046
258,0.7978968485,0.9916613418,0.8174654638
259,0.7987548345,0.9915934625,0.8179780469
260,0.7990182467,0.9918369915,0.8163339915
261,0.7993361454,0.9918357097,0.8151161519
262,0.7994916985,0.9918517037,0.8183397766
263,0.7982083877,0.9920773234,0.8175498277
264,0.799317973,0.9918437145,0.816026431
265,0.8002565631,0.991955923,0.8156398632
266,0.7984763568,0.9918440344,0.8169048208
267,0.7999300654,0.9917760661,0.8154518487
268,0.799149979,0.9919590789,0.8171535426
269,0.801244237,0.9917854187,0.8160788897
270,0.7995941906,0.9916135589,0.8167906302
271,0.8003144897,0.9919150235,0.8160153028
272,0.799467845,0.9915718423,0.8152397658
273,0.798687884,0.9917989261,0.8174654971
274,0.7990660193,0.9917969992,0.8151647948
275,0.7972372654,0.9918622254,0.8149936309
276,0.7980355914,0.9916832088,0.8168515759
277,0.7976973327,0.9917446142,0.8178955891
278,0.799443749,0.9917934641,0.8201889635
279,0.7990482374,0.9918072655,0.8168546668
280,0.7982167377,0.9919745071,0.8160167831
281,0.7969038167,0.9915751372,0.8169023477
282,0.7980019371,0.9918130291,0.8164012385
283,0.7969592291,0.9916942617,0.8156584118
284,0.7981023943,0.9916858121,0.8161658114
285,0.7991621606,0.9917488113,0.8157753122
286,0.7986057806,0.9915256663,0.8173897376
287,0.7987547231,0.9915784295,0.8154802644
288,0.8001513145,0.9917030181,0.8148070594
289,0.7990783358,0.9915896041,0.8164250823
290,0.7980689081,0.9915316187,0.8167343268
291,0.797591415,0.9917658786,0.816215405
292,0.7980374962,0.9914779674,0.8162149776
293,0.7985646793,0.9918895185,0.8158049326
294,0.798647652,0.9916511853,0.8167343268
295,0.7983499822,0.9915405318,0.8142873357
296,0.79684215,0.9917751874,0.8153989186
297,0.7981044496,0.9914277221,0.8155138742
298,0.7982128156,0.9916115382,0.8156992457
299,0.7971089446,0.9917153106,0.8155231999
300,0.798104706,0.9916648431,0.8147770987

==> tables/notation.tex <==
\begin{table}[ht]
\caption{Notation Table - \cuong{This table is defined but never cross-referenced. And since all the notations are already defined in the text, the table becomes unnecessary}}
\label{table:notation}
\begin{tabular}{cl}
\hline
Symbol & Description \\
\hline
$X$ & Instance space \\
$Y$ & Label space \\
$\Tilde{D}$ & Training set with noisy labels \\
$(\mathbf{x}_{i}, \hat{\mathbf{y}}_{i})$ & Pair of instance and its noisy label in the training set \\
$\mathbf{x}_{i}$ & Instance in the training set \\
$\mathbb{R}^{d}$ & d-dimensional real space \\
$\hat{\mathbf{y}}_{i}$ & Noisy label of the instance \\
$C$ & Number of classes \\
$\{0,1\}^{C}$ & Binary representation for C classes \\
$\pmb{1}$ & Vector of ones \\
$h_{\gamma}$ & Classifier parameterized by $\gamma$ \\
$\Gamma$ & Space of parameters for the classifier \\
$\mathbb{R}^{D}$ & D-dimensional real space for classifier parameters \\
$\Delta_{C-1}$ & \((C - 1)\)-dimensional probability simplex \\
\hline
\end{tabular}
\end{table}

